The Reality of the Situation: A Survey of Situated Analytics

The advent of low cost, accessible, and high performance augmented reality (AR) has shed light on a situated form of analytics where in-situ visualizations embedded in the real world can facilitate sensemaking based on the user's physical location. In this work, we identify prior literature in this emerging field with a focus on situated analytics. After collecting 47 relevant situated analytics systems, we classify them using a taxonomy of three dimensions: situating triggers, view situatedness, and data depiction. We then identify four archetypical patterns in our classification using an ensemble cluster analysis. We also assess the level which these systems support the sensemaking process. Finally, we discuss insights and design guidelines that we learned from our analysis.

==> appendices.tex <==
\newpage
\setcounter{page}{1}
\appendix

\begin{center}
  \huge{Supplemental Material: Sensemaking In Situ}
\end{center}

\section{Classification: Keshif Browser}

We have made our technique classification (Section~\ref{sec:design-space}) publicly (and anonymously) available in a Keshif~\cite{yalcin18keshif} browser: \url{https://explore.keshif.me/5681640172945408/5696764296298496/Situated_visualization}


==> backups/02_background_original.tex <==
\section{Background}
\label{sec:background}

Here we provide a background on immersive technologies, immersive analytics systems, and, in particular, situated analytics.
We begin by reviewing popular examples of situated visualization that are already in existence.

\begin{figure}[tbh]
    \centering
    \subfloat[A Navdy wayfinder shown on a car heads-up display.
    Image courtesy of Automotive Rhythms on Flickr (CC BY-NC-ND 2.0).]{
        \includegraphics[height=2.66cm]{figures/navdy-wayfinder}
        \label{fig:navdy-wayfinder}
    }
    \hspace{0.03in}
    \subfloat[Google Glass Explorer Edition.
    Image courtesy of Dan Leveille (CC BY-SA 3.0).]{
        \includegraphics[height=2.66cm]{figures/Google_Glass_photo}
        \label{fig:google-glass}
        
    }
    \caption{Examples of AR devices used for situated analytics. }
    \label{fig:ARdevices}
\end{figure}

\begin{figure}[tbp]
    \centering
    \subfloat[Virtual pens forming bars.]{
        \includegraphics[height=3.25cm]{figures/marvist-1.png}
        \label{fig:marvist-1}
    }
    \hspace{0.01in}
    \subfloat[Stacked glyph charts in an office.]{
        \includegraphics[height=3.25cm]{figures/marvist-2.png}
        \label{fig:marvist-2}
    }
    \caption{Examples from the MARVisT environment~\cite{chen19marvist}.}
    \label{fig:marvist}
\end{figure}

\subsection{Examples of Situated Visualizations}
\label{sec:archetypes_situatedvis}

There exist numerous instances of situated visualization in task-assisting applications, in popular games, and as concepts in science fiction.
Here we review some typical examples, real and imagined:

\begin{itemize}

\item\textbf{Heads-up displays} are mostly used for presenting information about the location and for providing simple instructional guidance (instructional) that overlay information on top of the user's field of vision. 
\textit{Examples:} military aircraft, high-end cars~\cite{kim18collisionar}, T-800 and T-1000 in the \textit{Terminator} movies, many 3D first-person games (\textit{Doom}, \textit{Elder Scrolls} series, \textit{World of Warcraft}). 
    
\item\textbf{Wayfinders/navigational aids} aid the user's movement around the physical world using contextual information, typically with specific final destinations in mind. 
The user's geographic information in the space is required, but features of the view are not necessarily embedded; in fact, many wayfinders use separate views.
However, some recently developed navigational aids utilize 2D or 3D embedded views (a design dimension we will explicate in Section~\ref{subsec:design_dimensions}). 
\textit{Examples:} Google Maps, Waze, Garmin GPS, Navdy (Fig.~\ref{fig:ARdevices}(a)), Google Live View.

\item\textbf{Embedded virtuality} integrates virtual objects into real-world scenes with the purpose of making the computer-generated imagery look real, or at least as if it belongs in the scene.  
\textit{Examples:} Simulation of technical details for expert use~\cite{doil03armanufacture}, virtual representation of a furniture into a room, or a place~\cite{gomez08sizeestimation}, augmented reality games (ARGs) such as Pok{\'e}mon GO~\cite{paavilainen17pokemongo}, visualization for underground construction sites~\cite{schall09infravis}.

\item\textbf{Embedded abstract information} focus on the integration of abstract information with real-world objects and points of interest in the user's view.
These systems tend to have 2D or 3D embeddings and are not quite as concerned with making the computer-generated imagery look real, but may try to do so. 
\textit{Examples:} Dominikus Baur's ``silent augmented reality'',\footnote{\url{https://do.minik.us/blog/silent-augmented-reality}} Quantic Dream's \textit{Heavy Rain} where Norman Jayden uses AR glasses to assist crime scene investigation, examples from the MARVisT system~\cite{chen19marvist} (Fig.~\ref{fig:marvist}), augmenting static visualizations with virtual content~\cite{chen20staticvis}.

\end{itemize}

\subsection{Immersive Technologies}

Immersive analytics is a rapidly developing area of research.
The three main types of immersive technologies are (1) \textit{virtual reality (VR)}, (2) \textit{augmented reality (AR)}, and (3) \textit{mixed reality (MR)}.
As of yet, there is no solid definition on these terms.
To avoid ambiguity, we only provide a brief introduction on these terms that we use in this paper, as discussing the differences between them in detail is out of scope of this work:

\begin{itemize}
    \item\textit{Virtual reality} is a computer-generated artificial environment that is separate from the real world.
    It is typically accessed using HMDs such as Oculus Quest, HTC Vive, and Samsung Gear (but also physical environments such as CAVEs as well as standalone ``fishtank'' VR displays). 
    
    \item\textit{Augmented reality}~\cite{azuma97AR} is a variation of virtual reality composed of virtual objects with the real world.
    AR environments have the following three characteristics: (1) combines real and virtual, (2) interactive in real time, and (3) registered in three dimensions. 
    
    \item\textit{Mixed reality}~\cite{chen17urbananalytics} refers to AR applications where real and virtual objects and scenery interact in a realistic manner.

\end{itemize}

Ever since Milgram et al.~\cite{Milgram1995} first outlined the continuum of interaction spaces ranging from reality to virtuality, the concepts of AR and VR and the relationship between them has become clearer.
While overly hyped decades ago, recent years have seen technological advances in both VR and AR that now finally promise to deliver upon their vast potential at the consumer level~\cite{Schmalstieg2016}.
Technologies now available for creating AR and VR environments are mainly split into physical installations, such as CAVE environments that project information and track users in a physical space~\cite{Raskar1998}, and wearable hardware that add a virtual (or simulated) information to the users's senses, including visual (first envisioned by Sutherland in 1968), auditory, somatosensory, and even olfactory senses~\cite{Paneels2010, Patnaik2019}.

Augmented and mixed reality are less well-explored than VR, but no less powerful.
The idea in AR and MR is to overlay the user's view of the real world with computer-generated contextual information.
However, while technology is improving, many challenges remain~\cite{Schmalstieg2016}, such as interaction, registration, calibration, tracking, and visual coherence.

\subsection{Immersive Analytics}

Recent work has proposed the notion of \textit{immersive analytics}~\cite{Marriott2018}, which Bowman et al.~\cite{bowman03richvirtual} refer to as \textit{information-rich virtual environments}: the use of data visualization in immersive visual environments.
However, using 2D visualizations in immersive settings is challenging; several frameworks have been developed to explore methods for visualization placement and interactivity within such immersive information spaces~\cite{park18graphoto, kwon16immersgv}.
3D visualization, on the other hand, while initially popular in the research field~\cite{Robertson1991}, has more recently been shunned in visualization research because of inefficiencies arising from occlusion, distortion, and navigation~\cite{Elmqvist2008, munzner14visualization}.

A new generation of virtual reality devices---especially at the consumer level---has made immersive technologies more accessible and powerful, and thus less affected by these factors~\cite{bach16immersiveanalytics, lee19immersive}. 

\subsection{Immersive Analytics in Virtual Reality}

The resurgence of virtual reality has led to a proliferation of immersive analytics tools in recent years.
Marai et al.~\cite{marai19immeleclesson} provide a history of immersive analytics tools for collaborative environments at the Electronic Visualization Laboratory (EVL) at University of Chicago.
Cordeil et al.~\cite{cordeil17immersivecollab} propose a multiuser system for visualizing collaborative graphs.
ImAxes is a virtual reality system based on 3D hand gestures to build multivariate visualizations~\cite{cordeil17imaxes}.
HeloVis~\cite{cantu18helovis} tackles large-scale display of data in 3D using helical shapes.
Bonada et al.~\cite{bonada16personimmersiv} work on personalizing views on immersive analytics via eye-tracking technology.
The Visualizer~\cite{billen083dgriddatavis} is a VR-oriented visualization software developed to bridge the gap between the technological and algorithmic challenges that can arise when building the environment, as well as to understand the utility of the software.
FiberClay~\cite{hurter19fiberclay} is an immersive multidimensional visualization system for understanding dense and complex datasets. 
Cerfontaine et al.~\cite{cerfontaine16immersivegeo} discuss the advantages and the disadvantages on interaction tasks in head-mounted VR-based immersive analytics systems using geoscientific data.

One research theme focuses on toolkits for immersive analytics.
DXR~\cite{sicat19dxr} and IATK~\cite{cordeil19iatk} are Unity toolkits for data visualization in immersive environments. 
Recently, a web-based toolkit, VRIA~\cite{butcher20vria}, has been  proposed for developing immersive analytic systems. 
The web-based Vistrates~\cite{Badam2018} toolkit can also be used for such applications.

Another theme studies user experiences in immersive analytics realized using virtual reality. 
Simpson et al.~\cite{simpson17take} assess the movement of scatterplots on an immersive environment.
Hube and M{\"u}ller~\cite{hube18data} suggest novel ways to project scatterplot and parallel coordinates onto a 3D virtual reality environment.
Batch et al.~\cite{batch20econimmersive} evaluate the effectiveness of immersive analytics for analysts in a year-long deployment at an economics government agency.
Kraus et al.~\cite{kraus20clusteridenttask} compare cluster identification tasks of scatterplots in various environments (i.e., screen 2D, screen 3D, VR table, and VR room), and concludes that the VR room is the most effective for the task.
Filho et al.~\cite{filho20spacetimegeovis} study spatiotemporal trajectories in geoographic spaces using a three-dimensional VR environment.
Finally, Ivanov et al.~\cite{ivanov19awalkamongthedata} conduct an experiental study on immersive visualization in a VR environment.

\subsection{Immersive Analytics and Mixed/Augmented Reality}

Augmented reality enables immersive analytics to be more integrated with the real world.
Luboschik et al.~\cite{luboschik16spatialperception} discusses common visual cues that help the spatial perception of datasets in AR-based immersive environments.
B{\"u}schel et al.~\cite{buschel173dvisualization} study 3D spatial interaction using mobile devices, as well as
the effectiveness of different edge types (e.g., curved, dashed, and straight) in a 3D augmented reality setting~\cite{buschel19argraphvis}.
Engelke et al.~\cite{engelke17qualityholobee} investigate the user experience of HoloBee~\cite{engelke16melissar}, a visual analytics system for analyzing bee drift data in AR.
Chen et al.~\cite{chen17urbananalytics} develop design spaces for urban immersive analytics.
The ``Hologram in my Hand'' by Bach et al.~\cite{bach18hologram} provides insightful information on the efficiency of various interaction tasks for different devices, including a Microsoft HoloLens, a mobile tablet, and a traditional desktop. 
MARVisT~\cite{chen19marvist} provides a novel technique for creating glyphs on an AR environment.
Langlotz et al.~\cite{langlotz14arbrowser} provide advice on how to design AR in a web browser from a computational perspective.
The paper also discusses limitations for AR technology in web browsers. 
Yang et al.~\cite{yang19flowmaps} develop MapsLink to compare the efficacy of visualizations between flat map and a 3D globe map. 

However, all of these examples so far are \textbf{not} situated in the actual physical space where the data is located, collected, or leveraged.
For that we turn to the concept of situated analytics.

\subsection{Situated Analytics}


\textit{Situated Analytics} (SA) is an emerging field where, according to Elsayed et al.~\cite{elsayed15situateddef}, analytical reasoning is supported by embedding the visual representations and interaction of the resulting data in a physical environment using augmented reality.
To make the distinction between SA and ``mere'' immersive analytics in augmented reality, as discussed in the prior section, we typically think of situated analytics as also requiring (1) a mobile platform, as well as (2) data that is tied to the specific physical location~\cite{Thomas2018}.

One of the earliest situated analytics systems is the Touring Machine~\cite{feiner97touringmachine}.
The user wears a see-through, head-worn display that is attached to a backpack.
Labels for campus buildings are then overlaid on top of the real-world environment.
The user can select any label to see detailed information about the building on a hand-held display. 

The real impact power and potential for situated analytics arises when supporting experts in the field.
A review paper by Behzadan et al.~\cite{behzadan15reviewarconstruction} surveys methods to blend data into AR displays on construction sites (e.g., creating views of underground utilities).
A more recent example of this marriage of data and reality is seen in FieldView~\cite{whitlock20fieldimmersive}, an AR-based immersive analytics system to help support the activities needed by domain experts working in the field. 

The ubiquity and compactness of mobile devices now offer the opportunity to collect, view, and analyze geospatial information in-situ~\cite{Lane2010, Zheng2014} to enhance the user's abilities to make spatial decisions~\cite{Andrienko2007}.
SiteLens~\cite{white09sitelens} uses handheld augmented reality through a mobile device to aid urban designers gain better insights by embedding relevant data in the city landscape.
Schall et al.'s underground infrastructure visualization~\cite{schall09infravis} draws underground utilities on top of a construction site or road to helps field workers in utility companies.
Additional situated analytics systems are designed for standard smartphones, such as for shopping~\cite{abao18foodgo, elsayed15situateddef} and tourism~\cite{williams17toarist, alqahtani17imapcampus}.

While surveys of AR applications in general~\cite{van10survey} and SA applications specifically~\cite{willett17embedded} may exist, our work is novel in that it provides a fine-grained analysis of dimensions along which can be used to closely evaluate them and understand the relationships between them.


\subsection{A Survey of Surveys}
\label{sec:survey_of_surveys}
There have been a number of surveys on AR and immersive analytics, both being domains that are heavily related to situated visualizations. 
We discuss a selection of related works.

First, we provide survey papers that discuss mainly on AR techniques. 
A number of papers discuss various applications, and provide advantages as well as challenges that needs to be addressed.
Azuma~\cite{azuma97AR} provides examples of applications and describes the differences between optical and video blending approaches in deploying augmented reality techniques. 
He also mention two big bottlenecks for effective augmentation of the real world: (1) accurate registration of a virtual object's location and (2) errors in sensing of the user's location and her surroundings. 
These two points are all related to accurately positioning the location of objects. 
Zhou et al.~\cite{zhou08artracking} discuss AR techniques that have been studied for a 10-year period starting from 2008 confined to the ISMAR conference. 
It discusses techniques in 3 main parts, (1) tracking techniques, (2) interaction techniques, and (3) display techniques, and describe the limitations from them. 
10 years later, Kim et al.~\cite{kim18arsurveyismar} provide a follow-up paper and describe major development of the existing AR techniques compared with those of the past 10 years. 
Van Krevelen and Poelman~\cite{vankrevelen10arapplications} introduce a variety of applications about AR systems in a detailed manner.
They point out other limitations of AR systems such as its use in outdoor, portability issue, depth perception, and over-reliance of information. 
Carmigniani et al.~\cite{carmigniani11arsurvey} distinguish AR systems into fixed/mobile indoor/outdoor/both indoor and outdoor systems to investigate how AR techniques would develop. 
They argue that successful mobile AR systems need to be fashionably and socially acceptable to be popularly accepted by the audience so that users can focus on applications, and less disturbed by computing devices. 
Another group of research have begun to describe specific areas (e.g., assembly plants~\cite{wang16ARcomprehensive}) and techniques (e.g., tracking technique~\cite{rabbi13survey} where AR is used as a key technique. 

In visualization community, systems that represent information related to its physical location have been introduced as a branch of immersive analytics systems~\cite{fonnet21iasurvey}. 
They analyze IA systems from 4 main perspectives: (1) technologies, (2) data mapping, (3) interactions, (4) collaboration, and (5) types of user studies conducted. 
They also propose three directions for the future of immersive analytics: (1) fostering multi-sensory and embodied interactive IA, (2) converge towards best practices, and (3) aim at real life IA systems. 
Willett et al.~\cite{willett17embedded} specify and define novel concepts such as embedded/situated data representation. 
They provide examples, compare and contrast between the representations, and provide future scenarios about them. 

Recently, Ens et al.~\cite{Ens2021} provide grand challenges to immersive analytics, and one of the topics is the `spatially situated data visualization.' 
They provide 5 challenges that persist in the topic. 
In our work, by discovering existing patterns and trends in the design of situated visualizations, we plan to mainly address the C3 of the challenges--- `designing guidelines for spatially situated visualisation.' 
% By 

==> backups/03_desing_space_OLD.tex <==
\section{Design Space: Situated Visualization} % with AR techniques}
\label{sec:design-space}

%Two major contributions of this paper are, first, our taxonomy for evaluating situated analytics literature, and second, our construction of a design space for situated visualization. 
%While this is clearly not a new research topic, as our literature survey shows, we are unaware of any existing structured exploration of this space. 

We describe our survey methodology for situated visualizations based on our meta-analysis of relevant work. 
We introduce our rubric for the selection of situated visualizations that use AR techniques. 
We collect relevant research works in a keyword-based search manner based on the rubric from a wide range of venues across various domains, and are not restricted to HCI, visualization, and AR/VR. 


\subsection{Collection of Papers for the Survey}
\label{sec:requirements}

% introduce about Bressa et al's paper
% Our definition + metrics.

The concept of situated visualization has been mentioned by researchers in the past, but the definitions about the concept has been diverging by researchers.
Bressa et al.~\cite{bressa:hal-03319648} surveyed about different definitions that have been used for situated visualizations. 
In our work, we refer to the definition of situated visualization by Willett et al.~\cite{Willet2017_Embedded} as ``\textit{place the entire visualization in a relevant location, but do not necessarily physically align individual data presentations or visual marks with their corresponding reference.}''
The selection of relevant SA and SV is determined using the definition by Willet et al.


\subsection{Survey Methodology}
\label{subsec:data_collection}

% collection of the corpus
% - Recent conferences --  going through list of papers that have situated visualization and augmetned reality
% - more than 5 years old -- depended on keyword search in venues. 
% - read the papers fully, and find out if they were relevant to the definition of situated visualization based on Willett et al. 
% 

We searched papers from academic literature within immersive technologies (VR, ISMAR, VRST, etc.), visualization (VIS, Eurovis, PacificVis, etc.) and human-computer interaction (CHI, UIST, AVI, etc.) for the past two decades.
The selection process is done by three of the researchers, and is selected as a relevant paper only if all three researchers agreed that the work is either a SA or SV. 

Initially, we ran into the lists of all papers in conferences of premier venues of immersive technologies (IEEE VR, ACM/IEEE ISMAR), HCI (ACM CHI), and visualization (IEEE VIS, IEEE TVCG). less than three years old and searched for papers that utilize situated visualizations.
For paper that are more than three years old, we conducted keyword-based search in different publisher websites (ACM Access, IEEE Access, Science Direct, and Elsevier).
We used the keywords that are related to SA and SV. 
Examles of these keywords are: `situated visualization,' `situated analytics,' `situated visualization with augmented reality,' `augmented reality visualization' and `situated visualization with AR.'

This yielded a total of 63 papers. 
The earliest work we add in our taxonomy is the Touring Machine~\cite{feiner97touringmachine} by Feiner et al., published in 1997. 
The distribution of the papers are shown in Table~\ref{table:summary_table}. 

% state how many are from VIS, HCI, AR/VR conferences
% situated visualization are used in various domains ... 
% Various form factors (...)
% 



%In our survey of surveys (Section~\ref{sec:survey_of_surveys}), we \textbf{[...finish meee...]}

% We believe that our selection criteria are justified because \textbf{[...finish meee...]} --- I think that this is explained in the related work. 

\begin{comment}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figures/sac_origin.eps}
    \caption{\textbf{Temporal evolution of situated visualizations by origin.}
    Increasing trend as the number of visualizations increase.}
    \label{fig:stat_paper}
\end{figure}

\end{comment}

\subsection{Design Dimensions}
\label{subsec:design_dimensions}


We identify four primary dimensions for situated visualizations, and evaluate the literature in our survey along these and five additional secondary dimensions common throughout visualization literature in general (situated or otherwise).
This task is done between all of the authors. 


% Discuss issues about problems with existing taxonomies in visualization. What it does not collect. 
% Data types according to Ben Shneiderman (There are some types that do not need this)
% Tasks, purposes in InfoVis literature (Some don't even fall under the category)
% However, technologies in AR are not limited to a canvas, and a dashboard --- the advancements in form factors bring different visualization. They involve a more authentic experience, take advantage of being in the place, and require different types of cues to represent the data. 

% Hence, this needs different design space. 

% Why is it important to conduct a survey on techniques? 
% Combination of different 

The main focus of the techniques is to identify how techniques are used in the inter-relationships between the device, the user, and the visualizations within the view. 
In the recent survey by Bressa et al~\cite{bressa:hal-03319648}, they provide provide 7 elements for the dimension `technology.' These are: AR, VR, physicalization, analog, display, mobile device, and others. 
Such taxonomy of techniques is a mixture of techniques and form factors that does not comprehensively represent the concept of `technology' used for SA and SV. 
For example, AR/VR and physicalization are means to present data in SV, while mobile device and display are form factors that are used in SA.
Such irregular criteria in the elements of technology make it difficult for the audience to recognize the technical characteristics of various systems. 
To address such issues and study deeper into SA/SV, we mainly focus on taxonomizing the techniques of SA/SV that utilize AR in particular, because not only is it frequently deployed in SVs, but is also a rapidly evolving technique that is gaining wide interest from researchers. 

To begin with, we observed four technical specifications of situated visualizations that utilize AR techniques. 
These are: (1) form factors used to present the system (e.g., mobile, head-mounted, world, etc.), (2) integration techniques used to present data within the user's view (e.g., separate, overlay, 2D-, 3D-, non-visual, etc.) (3) interaction techniques that users use to interact with the system (e.g., touch, pen, gestural, etc.), and (4) navigation techniques used to change the view of the system (e.g., location, gaze orientation etc.). 

Then, based on these observations, we found dimensions that could not only fit these systems but also thoroughly explain each systems' qualities that pertain to the user, situatedness, and presentation of the data. The four dimensions and the values corresponding to each one are:

\begin{enumerate}
    \item\textsc{Situating Triggers:} Discrete events that lead to the instantiation or modification of a situated visualization.
    \begin{itemize}
    
        \item\textbf{Referents:} Spatial triggers that indicate a view should be instantiated or modified.
        
        \begin{itemize}
            \item\textit{Location:} When the instantiation of the data view or visualization is triggered by the user's location; in contrast with context, this may not be a semantic place (e.g., GPS location, or distance walked from scene starting point in steps as indicated by pedometer). 
            
            \item\textit{Object:} When the instantiation of the data view or visualization is triggered by an object being detected by a sensor or camera on the user's device (e.g., marker, object recognition, loud sound originating near the user).

        \end{itemize}

        \item\textbf{Context:} When the instantiation of the data view or visualization is triggered by semantic or conceptual information surrounding the user at the current time and place.
        The trigger may or may not be spatial.
        Types of context situating triggers include:
        
        \begin{itemize}
            \item\textit{Timely events:} Cross-sectional information about actions identified at a moment in time as falling within scope of a view.
            These events can be planned to occur at a known point in time (e.g., someone calls me to schedule a meeting, and a timer is added to my view when the meeting is ten minutes from starting).
            They can also be unplanned: this includes situational information identified by the system at a given moment in time that triggers a view instantiation or modification (e.g., a fight breaks out near the user).
            
            \item\textit{Specific setting:} The type of space that the user is in and its state at the time they are in it (e.g., mesh/topological map of the environment being classified as, for example, a construction site; referent is the user and the user’s desires, in contrast with object and location).
            
        \end{itemize}
            
        \item\textbf{Non-situated:} The command for the creation of the view is user-driven independent of the user’s locus, context detected by the system, or objects in the view of system sensors.
        %For example, assume a user wants to look at their parking spot and requests a view, but a view cannot be created in situ without the system identifying the appropriate positioning of the view, which requires a situated trigger.
        A system may have a non-situated view creation command, but in order for a view to be situated--i.e., positioned relative to objects, locations, or contexts around the user--a situating trigger is still required.
        If neither the trigger nor the view are situated, the system is not a situated analytics system.
        Consequently, non-situated systems have not been included in Table~\ref{table:summary_table}.
    \end{itemize}
        
    \item\textsc{View Situatedness}: The layout of data views as linked to the world around the user, potentially including their device's viewport.
    
    \begin{itemize}
    
        \item\textbf{World-Registered:} When the data is presented in a way that is positionally anchored to the real world, such as an imitation of a real object (e.g., an amount of stacked sugar cubes representing the amount of sugar in food items sitting on a table near those food items).
        
        \begin{itemize}
            
            \item\textit{World-absolute:} the data is situated at the exact point of interest (e.g., a holographic representation of a person to reenact an event exactly on top of a marker).
            
            \item\textit{World-relative:} The data is situated in a location that is relevant to a given point of interest, but the actual layout of the visualizations is designed to optimize user interpretation of the information rather than to strictly mirror real world object positions or location (e.g., a cluttered real-world view with labels that are neatly organized but linked to real world objects via curves).
                
        \end{itemize}
            
        \item\textbf{Sticky:} data is situated at the exact point of interest (world-registered) until it moves out of the field of view.
        Then it appears at the periphery of the view, becoming device-anchored (device-relative).
        
        \item\textbf{Device-Anchored:} the data is situated at a location not necessarily visually linked to the given point of interest, but is still part of a situated system due to the situating trigger causing the view to be instantiated.
        E.g., a popup notification on a smartphone when you are near a point of interest.
        
        \begin{itemize}
        
            \item\textit{Device-fixed (Overlay):} When the data is represented in front of the user’s view of the real world on their device, without being registered to the world (e.g., a heads-up display, or a HUD reticle).
            This definition is comparable to the usage of the same abbreviation for Cascading Stylesheets (CSS) in modern web design.
            
            \item\textit{Device-relative:} When the data is presented in a way that is not fixed in the user's field of view, but is anchored to the user (e.g., the view is inside a window or multiple windows always positioned to the south of the user, or a GPS map on a smartphone that rotates and changes based on the user's position and orientation)%, the view is rendered on the screen of a mobile device).
            %Example: HUD reticle - World-registered but device-anchored?

        \end{itemize}

        \textit{Special note}: A view can be both absolute and relative: An object may be positioned absolutely inside an automobile, for example, but the automobile is a container with a moving position and as such the position of the view is relative to the automobile. These definitions are comparable to the CSS usage of the same words.
    \end{itemize}
    
    \item\textsc{Data Depiction:} The physical form that data representations take; i.e., the visual encodings of data features.
    
    \begin{itemize}
    
        \item\textbf{2D:} Data is depicted on a two-dimensional plane.
        
        \item\textbf{3D:} Data is depicted as a three-dimensional entity.
        
        \item\textbf{Non-visual:} The data is depicted in a non-visual manner (e.g., sound, smell, etc.).
        
    \end{itemize}
    
    \item\textsc{Data Abstraction:} Visual Expressions used for data representations.
    
    \begin{itemize}
    
        \item\textbf{Abstract:} the data is expressed in graphical marks and channels that are used to encode features and values of a dataset (e.g., lines, squares, spheres, etc. of varying color, position, size, etc.).
        
        \item\textbf{Physical:} the data is expressed using the real world's spatial dimensions to represent spatial features of the data. 
        
        \begin{itemize}
            
            \item\textit{Simulated:} the data/entity is expressed as a computational imitation of an existing object/entity (e.g., a heart positioned in a cutaway over a human patient).
            
            \item\textit{Map:} a representation of a space or place, rescaled for user overview of surroundings (e.g., world-in-miniature (WIM), 2D map canvas).
            
        \end{itemize}
        
    \end{itemize}
    
\end{enumerate}

\begin{comment}
\begin{figure}[tbp]
    \centering
    \includegraphics[width=250px]{figures/dimension_instruction_3.png}
    \caption{A diagram to represent the relationship of the four dimensions with the world, data, and user's view. (1) The world triggers the visualization (situating triggers). Then, (2, 3) relevant data is chosen for presentation. With appropriate choice of data abstraction and data depiction, (4) the view is presented to the user around the world (view situatedness).}
    \label{fig:dimensions-diagram}
\end{figure}
\end{comment}
\subsection{Survey Corpus}

Based on the dimensions and collected papers, we created a table to present each SA based on our taxonomy in Table~\ref{table:stats_table}.
%As a slight summary of our taxonomy, we provide the frequency ((( add a rough summary about the taxonomy in terms of numbers and charts ))).

%- stuffs to provide 
%%- a bar chart showing temporal trends.
%- a small table to show in 



\newlength{\Oldarrayrulewidth}
\newcommand{\Cline}[2]{%
  \noalign{\global\setlength{\Oldarrayrulewidth}{\arrayrulewidth}}%
  \noalign{\global\setlength{\arrayrulewidth}{#1}}\cline{#2}%
  \noalign{\global\setlength{\arrayrulewidth}{\Oldarrayrulewidth}}}



\begin{table*}[]
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\caption{Taxonomy of research works that utilize AR techniques for situated visualizations. }
\label{table:summary_table}
\vspace{-0.1in}
\centering
\sffamily
\tiny
\resizebox{\textwidth}{!}{%

\setlength\arrayrulewidth{0.5pt}

\begin{tabular} {|l|rr|c|c!{\color{diagramGrey}\vrule}c|c!{\color{diagramGrey}\vrule}c|c!{\color{diagramGrey}\vrule}c|c|c!{\color{diagramGrey}\vrule}c|c!{\color{diagramGrey}\vrule}c!{\color{diagramGrey}\vrule}c|c!{\color{diagramGrey}\vrule}c!{\color{diagramGrey}\vrule}c|}
\cline{5-19}
% {|m{2cm}|m{1ex}|m{1ex}|m{1ex}}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{|c|}{situating triggers} & \multicolumn{5}{c|}{view situatedness \vspace{0.02in}} & \multicolumn{3}{c|}{ data  } & \multicolumn{3}{c|}{ data }  \\ \cline{5-13}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{|c|}{referents} & \multicolumn{2}{c|}{context} & \multicolumn{2}{l|}{  device-} & \multicolumn{1}{c|}{} & \multicolumn{2}{l|}{world-} & \multicolumn{3}{c|}{depiction} & \multicolumn{3}{c|}{abstraction} \\
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{l|}{anchored} & \multicolumn{1}{c|}{} & \multicolumn{2}{l|}{registered} & \multicolumn{3}{l|}{} & \multicolumn{3}{l|}{} \\ \cline{5-10} \cline{12-19}
\multicolumn{1}{c}{\textbf{n\textsuperscript{o}}} & \multicolumn{1}{c}{\textbf{name (shortened)}} & \multicolumn{1}{c}{\textbf{year}} & \multicolumn{1}{c}{\textbf{cluster}} & \multicolumn{1}{|c}{\rotatebox{90}{location}} & \multicolumn{1}{c|}{\rotatebox{90}{object}} & \multicolumn{1}{c}{\rotatebox{90}{timely}} & \multicolumn{1}{c|}{\rotatebox{90}{setting}} & \multicolumn{1}{c}{\rotatebox{90}{relative}} & \multicolumn{1}{c|}{\rotatebox{90}{fixed}} & \multicolumn{1}{c|}{\rotatebox{90}{sticky}} & \multicolumn{1}{c}{\rotatebox{90}{absolute}} & \multicolumn{1}{c|}{\rotatebox{90}{relative}}  & \multicolumn{1}{c}{\rotatebox{90}{2D}} & \multicolumn{1}{c}{\rotatebox{90}{3D}} & \multicolumn{1}{c|}{\rotatebox{90}{nonvisual}} & \multicolumn{1}{c}{\rotatebox{90}{abstract}} & \multicolumn{1}{c}{\rotatebox{90}{map}} & \multicolumn{1}{c|}{ \rotatebox{90}{simulated \vspace{-0.01in}} \hspace{-0.03in} }  \\

\hline
 
1 & A Touring Machine~\cite{feiner97touringmachine} & 1997 & C3 & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
%\arrayrulecolor{diagramGrey}\hhline{~|~|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
2 & Augmentable Reality~\cite{rekimoto98augmentable} & 1998 & C5 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
3 & Situated Documentaries~\cite{hollerer99sitdocument} & 1999& C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
4 & MARS~\cite{hollerer99mars} & 1999 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark \\
%%%%%
%\hdashline
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
5 & Information Filtering for Mobile AR~\cite{julier02info_filtering} & 2000 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
6 & AR for Military in Urban Terrain~\cite{livingston02augmented} & 2002 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
7 & AR for Manufacture Planning~\cite{doil03armanufacture} & 2003 & C1  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
8 & AR/VR in Digestive Surgery~\cite{soler04digestiveAR} & 2004 & C6  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
9 & AR on Molecular Models~\cite{gillet04moleculeAR} & 2004 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
%%%%%%
%\hdashline
\arrayrulecolor{diagramGreen}\Cline{0.3pt}{3-3}\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
10 & ARVino~\cite{king05arvino} & 2005 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
11 & AR for Construction~\cite{Behzadan05constructionAR} & 2005 & C1  & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
12 & Hypermedia Vis for AR/VR~\cite{guven06arhypermedia} & 2006 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
13 & AR on Historic Sites~\cite{guven06historicsitesAR} & 2006 & C1  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
14 & Focus and Context Vis for AR~\cite{kalkofen07ContextAR} & 2007 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
15 & AR for Size Estimation~\cite{gomez08sizeestimationAR} & 2008 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
16 & Situated Vis for Keyhole Surgery~\cite{bichlmeier09keyholesurgeryAR} & 2009 & C6  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
17 & Vis for Psychomotor-Cognitive Tasks~\cite{kotranza09psychomotorAR} & 2009 & C6  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
18 & SiteLens~\cite{white09sitelens} & 2009 & C1  & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark &  \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
19 & Underground Infrastructure Vis~\cite{schall09infravis} & 2009 & C7  & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
%%%%%%
%\hdashline
\arrayrulecolor{diagramGreen}\Cline{0.3pt}{3-3}\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
20 & AR for Opportunistic Controls~\cite{henderson10tangibleAR} & 2010 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
21 & AR with Paper Maps~\cite{morrison11papermapAR} & 2011 & C2  & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-18}
22 & Indoor Navigation AR~\cite{mulloni11indoorAR} & 2011 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
23 & AR for Maintenance and Repair~\cite{henderson11maintenancerepairar} & 2011 & C4  & \xmark & \cmark & \xmark & \xmark &  \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
24 & Bottari~\cite{bladuini12bottari} & 2012 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
25 & Label Placement in AR~\cite{grasset12viewmanagementAR} & 2012 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
26 & AR for Outdoor Navigation~\cite{dunser12ARoutdoornavigation} & 2012 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
27 & CityViewAR~\cite{lee12cityviewAR} & 2012 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
28 & Inattentional Blindness in Surgical AR~\cite{dixon13surgeons} & 2013 & C1  & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
29 & Orientation Measurement for Audio AR~\cite{heller14mobaudioar} & 2014 & C5  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
30 & Indoor Navigation Vis~\cite{moller14indoornavigation} & 2014 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
31 & In-Situ Climate Change Vis~\cite{liestol14climate} & 2014 & C6  & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
32 & Wind and Uncertainty Vis~\cite{fjukstad14weatherforecast} & 2014 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\ 
%%%%%%
%\hdashline
\arrayrulecolor{diagramGreen}\Cline{0.3pt}{3-3}\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
33 & Borehole AR~\cite{lee15boreholear} & 2015 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
34 & HMD Vis for the Deaf~\cite{jain15hmdvis} & 2015 & C5  & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
35 & In-Situ Flood Vis~\cite{haynes16floodAR} & 2016 & C1  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
36 & Horus Eye~\cite{elsayed16horuseye} & 2016 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark &  \xmark \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
37 & SA for Shopping~\cite{elsayed16situateddef} & 2016 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
38 & Crime Scene Investigation AR~\cite{datcu16csiar} & 2016 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
39 & Riverwalk~\cite{cavallo16riverwalk} & 2016 & C7  & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
40 & Pedestrian Navigation AR~\cite{joonagata17pedestrianAR} & 2017 & C2  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
41 & SonifEye~\cite{roodaki17sonifeye} & 2017 & C5  & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
42 & SA for Network Data~\cite{zhao17egocentricar} & 2017 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
43 & ServAR~\cite{rollo17servar} & 2017 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
44 & ToARist~\cite{williams17toarist} & 2017 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
45 & iMAP-CampUS~\cite{alqahtani17imapcampus} & 2017 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
46 & Cues for Social Contacts~\cite{nassani17socialcontactar} & 2017 & C7  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
47 & The Urban Cobuilder~\cite{imottesjo18urbancobuilder} & 2018 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
48 & FoodGo~\cite{abao18foodgo} & 2018 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
49 & Collision Warning AR~\cite{kim18collisionar} & 2018 & C3  & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
50 & MARVisT~\cite{chen19marvist} & 2019 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
51 & Clutter Management in AR~\cite{zhao19clutterar} & 2019 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
52 & Information Seeking Strategy in AR~\cite{caggianese19arinformationseek} & 2019 & C3  & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
53 & Situated Storytelling~\cite{ketchell19situatedstorytelling} & 2019 & C2  & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
54 & Agricultural Fieldwork Vis~\cite{zheng19fieldworkar} & 2019 & C2  & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
%%%%%
%\hdashline
\arrayrulecolor{diagramGreen}\Cline{0.3pt}{3-3}\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
55 & FieldView~\cite{whitlock20fieldview} & 2020 & C3  & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
56 & Usability of Augmented SV~\cite{guarese20augmentedsitvis} & 2020 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
57 & PapARVis~\cite{chen20staticvis} & 2020 & C5  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
58 & Corsican Twin~\cite{prouzeau20corsiantwin} & 2020 & C1  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
59 & Supporting Fine Details from AR~\cite{jiang20finedetailsar} & 2020 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
60 & HydrogenAR~\cite{whitlock20hydrogenar} & 2020 & C1  & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
61 & Basketball AR~\cite{lin21basketballar} & 2021 & C1  & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
62 & Impact of 2D Visualizations in AR~\cite{satkowski212darvis} & 2021 & C4  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
63 & Visualizing Air Pollution (AiR)~\cite{mathews21airpollutionvis} & 2021 & C2  & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark  \\
\arrayrulecolor{diagramGrey}\Cline{0.3pt}{4-19}
64 & MARVIS~\cite{langner21marvis} & 2021 & C2  & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark  \\
\arrayrulecolor{black}\hline
%\hline
\end{tabular}
}
\end{table*}

\begin{table*}[]
\def\arraystretch{1.1}%  1 is the default, change whatever you need
\caption{A statistical summary of information about the papers used in the taxonomy. Each value in the four dimensions are abbreviated in three/four letters. }
\label{table:stats_table}
\centering

\sffamily
%\resizebox{\textwidth}{!}{%
\resizebox{\textwidth}{!}{%

\begin{tabular}{c|ccccccc|cc|cc|ccc|ccc|ccccc|}

% {|m{2cm}|m{1ex}|m{1ex}|m{1ex}}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{} & \multicolumn{4}{c|}{situating triggers} & \multicolumn{3}{c|}{ data  } & \multicolumn{3}{c}{ data }  & \multicolumn{5}{|c|}{view situatedness \vspace{0.02in}}  \\ 
\multicolumn{1}{c}{} & \multicolumn{7}{c}{  } & \multicolumn{2}{c|}{referents} & \multicolumn{2}{c|}{context} & \multicolumn{3}{c|}{depiction} & \multicolumn{3}{c}{abstraction} & \multicolumn{2}{|l|}{device-} & \multicolumn{1}{c|}{} & \multicolumn{2}{l|}{world-}  \\
\multicolumn{1}{c}{} & \multicolumn{7}{c}{ Clusters } & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{3}{l|}{} & \multicolumn{3}{l}{} & \multicolumn{2}{|l|}{anchored} & \multicolumn{1}{c|}{} & \multicolumn{2}{l|}{registered}  \\ 
\multicolumn{1}{c}{\textbf{year}} &\multicolumn{1}{c}{\textbf{C1}} &\multicolumn{1}{c}{\textbf{C2}} &\multicolumn{1}{c}{\textbf{C3}} &\multicolumn{1}{c}{\textbf{C4}} &\multicolumn{1}{c}{\textbf{C5}} &\multicolumn{1}{c}{\textbf{C6}} &\multicolumn{1}{c}{\textbf{C7}} & \multicolumn{1}{c}{\rotatebox{0}{loc}} & \multicolumn{1}{c|}{\rotatebox{0}{obj}} & \multicolumn{1}{c}{\rotatebox{0}{time}} & \multicolumn{1}{c|}{\rotatebox{0}{set}} & \rotatebox{0}{2D} & \rotatebox{0}{3D} & \multicolumn{1}{c|}{\rotatebox{0}{nonv}} & \multicolumn{1}{c|}{\rotatebox{0}{abs}} & \multicolumn{1}{c|}{\rotatebox{0}{map}} & \multicolumn{1}{c}{ \rotatebox{0}{simu \vspace{-0.01in}} \hspace{-0.03in} } & \multicolumn{1}{|c}{\rotatebox{0}{rel}} & \multicolumn{1}{c|}{\rotatebox{0}{fix}} & \multicolumn{1}{c|}{\rotatebox{0}{sti}} & \rotatebox{0}{abs} & \multicolumn{1}{c|}{\rotatebox{0}{rel}}    \\

\hline

bef. 1999 & 0 & 0 & 3 & 0 & 1 & 0 & 0 & 3 & 0 & 0 & 1 & 3 & 3 & 1 & 4 & 0 & 1 & 0 & 4 & 0 & 4 & 0  \\
2000 - 2004 & 2 & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 2 & 0 & 2 & 3 & 3 & 0 & 3 & 0 & 2 & 0 & 2 & 0 & 4 & 1   \\
2005 - 2009 & 5 & 0 & 2 & 0 & 0 & 2 & 1 & 2 & 3 & 0 & 2 & 2 & 4 & 1 & 1 & 0 & 5 & 0 & 0 & 1 & 3 & 3   \\
2010 - 2014 & 1 & 5 & 2 & 3 & 1 & 1 & 0 & 6 & 6 & 0 & 3 & 11 & 2 & 1 & 11 & 5 & 4 & 5 & 5 & 2 & 6 & 0   \\
2015 - 2019 & 4 & 6 & 3 & 5 & 2 & 0 & 2 & 11 & 8 & 3 & 2 & 13 & 8 & 2 & 18 & 2 & 5 & 4 & 15 & 0 & 8 & 2   \\
2020 - onw. & 3 & 1 & 1 & 2 & 1 & 0 & 0 & 2 & 4 & 1 & 3 & 6 & 4 & 0 & 7 & 0 & 2 & 2 & 4 & 0 & 6 & 0  \\
\hline

\textbf{Total} & \textbf{15} & \textbf{12} & \textbf{12} & \textbf{12} & \textbf{5} & \textbf{4} & \textbf{3} & \textbf{25} & \textbf{23} & \textbf{4} & \textbf{13} & \textbf{38} & \textbf{24} & \textbf{5} & \textbf{44} & \textbf{7} & \textbf{19} & \textbf{11} & \textbf{30} & \textbf{3} & \textbf{31} & \textbf{6} \\

\hline
\end{tabular}
}

\end{table*}

==> backups/junk_applications.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%
%   NOTE: THIS SECTION IS NOT IMPORTED INTO THE FINAL MANUSCRIPT BECAUSE WE DO NOT WISH TO INCLUDE IT.
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Applications for Situated Analytics} 
\label{sec:applications}

Here we introduce 8 application areas where SA could be used---or is already being used---to great effect. The examples we provide in each area includes, but are not limited to academic works. 

\begin{itemize}

\item\textbf{Engineering:} Situated analytics can help technicians who are building and repairing complex machinery and circuitry by overlaying relevant schematics on their field of vision.
For example, an automobile mechanic may see an interactive schematic showing the different screws and bolts to remove in order to access and replace a broken part.
While these strictly speaking are not visualizations, the step to providing visual representations of data, such as for testing results or diagnostics, is not far.


\item\textbf{Construction:} Construction sites are also where situated analytics can benefit from. 
Visualizations for construction sites can provide an inner visualization of existing underground infrastructures (e.g., water supply facilities, sewerage system, etc.)~\cite{schall09infravis}, simulate construction design in real space~\cite{behzadan05constructionsim}, etc.). 
The early forms of situated visualizations for constructions are made using multiple form factors (e.g., a laptop computer at hand, a head-mounted display, and a GPS sensor mounted on the back). 
Recent works and applications are based on a simplified form factor (i.e., an electronic tablet).  

\item \textbf{Surgery:} Surgical procedures can be notoriously information-dense, requiring a doctor to combine multiple sources of information to make the correct decision. Furthermore, it can be a both mentally and physically enduring task, where visual assistance can be helpful.  
A situated analytics system for surgery support could overlay this data on top of the surgeon's field of vision~\cite{hbrsurgery}.%, as shown in Fig.~\ref{fig:medical-example}. 
Although this is still an aspirational goal, several prototype applications already exist.
Soler et al.~\cite{soler04surgery} provide markings to aid the digestive surgery of surgeons. The work by Bichleimer et al.~\cite{bichleimer09surgery} implement a see-through magic-lens to view the inner parts of human body for surgical purposes.  
Commercially, Kapanu~\cite{kapanu}, a spin-off from ETH Z{\"u}rich, provides an AR-based applications for dentistry that simulates how the patient's teeth are going to look after an operation. 

\item \textbf{Military:} Military aircraft have long used situated analytics through the use of fixed heads-up displays (HUDs)---which display vital information on the pilot's field of vision, thus reducing the need to look down (hence the name) at the instrument panel---since at least the 1950s, and newer aircraft use smart helmets where the augmented reality is embedded in the pilot's glasses.
The helmet rapidly provides information via standardized symbols to pilots so that they can quickly be aware of the threats and the situations surrounding the space~\cite{military_ex}. 

Because soldiers need to respond to unexpected situations instantaneously, the primary importance of a supporting device for them is ambidexterousness, as shown in the work by Livingston et al.~\cite{livingston02augmented}. 
The early form of situated systems have multiple form factors.
However, given miniaturized technology and improved batteries, such technologies are now beginning to reach individual soldiers on the battlefield.%; Fig.~\ref{fig:military-example} shows a mockup of such a personal situated analytics system. 

\item \textbf{Tourism:} Tourism can also take advantage of situated analytics. 
Large art museums such as Mus\'ee de Louvre and Mus\'ee d'Orsay provide an audio-based commentary about a work of art that is mapped to a particular number, or a fiducial marker. 
Tourist applications that share situated analytics techniques help tourists by providing relevant information about the situated location and by providing augmented user experience through the embedding of fictional objects. 
The advent of smartphones has allowed the invention of various types of situated visualizations for tourism~\cite{dunser12ARoutdoornavigation, cavallo16riverwalk}. 
A common type of tourist applications is those that provide information about the neighboring tourist destination~\cite{williams17toarist}.
These applications are usually presented in the form of map-sep-overlays (defined in Section~\ref{subsec:taxonomy_analysis_overview}) where the users can easily switch the views from map view and the information overlaid in camera view. 
Recent applications aim to provide new form of experience by taking advantage of embedded technologies.
For example, Riverwalk~\cite{cavallo16riverwalk} is a smartphone- and tablet-based application in which pointing the phone camera at a specific location superimposes a historical photograph of the same location on the device's live camera stream.

\item \textbf{Shopping:} Shopping applications that use situated analytics techniques to help customers have been developed to let users make rational choices by providing analytical capabilities.
Such applications include those that provide additional information (e.g., suggestion for a healthier choice), and make it convenient to make comparisons with other products. 
With the advent of AR technology on hand-held devices, customers can easily experience the product before purchasing it.
For example, IKEA Place, a new augmented reality app provided by IKEA~\cite{ikea_app}, allows the user to virtually place selected furniture in their own homes. 

\item \textbf{Driving:} Situated analytics can augment a person's driving experience.
Many vehicle manufacturers nowadays provide heads-up displays (HUDs) installed in their cars. 
Fig.~\ref{fig:ARdevices}(a) shows a third-party car-mounted HUD.
The HUD tells the driver about the car conditions (e.g., amount of gas, liquids, temperature) overlaid on the driver's windshield, and can even provide driving guidance (e.g., GPS navigation, lane guidance, blind-spot detection). 
Such guidance can enhance driver's performance~\cite{kim18collisionar}.  

\item \textbf{Architecture/urban planning walkthroughs:} Situated analytics can be advantageous in architecture and urban planning by enabling the situated instantaneous analysis of the environment. 
%Fig.~\ref{fig:building-example} shows a fictional situated analytics real estate application for augmented reality. 
The overlay of information and the analysis of such data will contribute to a better decision-making process. 

The simulation of the parts of a structure, or even the entire structure, in a real-world environment can help urban-planning experts assess the impact the structure would have. 
Other analysis tools could help assess the impact of a structure on its surroundings, such as predicting the impact of the structure on traffic, or its effect on natural lighting throughout the day and over the seasons~\cite{AR_urbandesign}.

\end{itemize}

%\begin{comment}

%\begin{figure}[tbp]
%    \centering
%    \includesvg[width=\columnwidth]{figures/ikea_place2.svg}
%    \caption{The IKEA Place app. Image Courtesy of Inter IKEA Systems B.V. 2019.}
%    \label{fig:ikeaplace-example}
%    \vspace{-0.2in}
%\end{figure}
%\end{comment}



==> backups/rubbish.tex <==
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003145</concept_id>
<concept_desc>Human-centered computing~Visualization</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003145.10011769</concept_id>
<concept_desc>Human-centered computing~Empirical studies in visualization</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003145.10011770</concept_id>
<concept_desc>Human-centered computing~Visualization design and evaluation methods</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Visualization}
\ccsdesc[500]{Human-centered computing~Empirical studies in visualization}
\ccsdesc[500]{Human-centered computing~Visualization design and evaluation methods}

%% Keywords
\keywords{Immersive analytics, situated analytics, augmented reality, mixed reality.}




\begin{comment}
\subsection{Tasks}

Based on the research literature and the above commercial applications, we identify 8 main tasks that people tend to perform using SA systems. 

\begin{itemize}
\item \textbf{Information exploration (undirected):} One task of situated analytics systems is providing contextual information about the location.
Google Maps, for example, automatically provides numerous types of information about the surrounding location (e.g., restaurants, gas stations, the shortest path to a destination).  

\item \textbf{Information seeking (directed):} Some situated analytics systems provide users contextual information for a specific purpose (e.g., highlighting the nutritional content of food products in a supermarket~\cite{abao18foodgo}).

\item \textbf{Notification:} Another common task found in situated analytics systems is drawing the user's attention to specific features in the environment, such as highlighting a radar contact on a military HUD (or on T-1000s field of vision), providing warnings when the user approaches a crime scene site, or flagging the arrival of an email in the user's inbox.

\item \textbf{Wayfinding (spatial navigation):} Wayfinding systems guide the user in physical navigation.
Advanced systems can even use information about the environmental, such as traffic, crime rate, and time of day, to provide the optimal route to the destination.

\item \textbf{Sensemaking (spatial sensemaking):} Sensemaking of spatial information is particularly useful in a situated setting, such as understanding walking patterns on a university campus, the impact of a new building on traffic, and the placement of buildings over time in a historic district.

\item \textbf{Narrative construction:} Specialized situated analytics systems can support storytelling activity of users (e.g., crime scene investigation) by combining the spatial information with the advantage of being in-situ~\cite{datcu16csivis}. 

\item \textbf{View arrangement:} Arranging 3D object and data in a real world environment provides users the opportunity to try activities that were difficult or impossible in 2D~\cite{imottesjo18urbancobuilder}, such as virtually testing a piece of furniture product in the users' living room~\cite{ikea_app}. %Fig.~\ref{fig:ikeaplace-example}.

\item \textbf{Memory and recall:} Humans have specialized spatial memory, allowing them to more easily memorize and recall information that can be placed in a spatial context~\cite{robertson98datamountain, radu14augmented}.

\end{itemize}
\end{comment} 


\subsection{Evolving Trends of Situated Visualizations}
\label{sec:temporal_trends}



%To summarize, situated visualizations are developing in a way that is `more ambidexterous, more sophisticated integration, more simplified form factor, more immersive, and more simplified interaction.' 

\subsubsection*{Ambidexterous situated visualizations.} A majority of the early sitauted visualizations tend to perform single task, mainly `learning' tasks. However, recent works can perform more than multiple tasks. The combination of analytical-learning and simulation-learning has led the increase of multi-functional situated visualizations. 

\subsubsection*{Sophisticated Integrations.} Another noticeable pattern from the data was that integrations into the user's view have become more manifold. The graph in Fig.(((((ADD HERE))))) shows that the  the number of situated visualizations are rapidly increasing, doubling approximately every XX years (((((make calculations))))). Integrations are more sophisticated than simple overlay (e.g., wim-sep-overlay) Furthermore, With the increased 2D, 3D embedded technology, the types of integrations have become more varied (e.g., overlay-2demb, overlay-3demb, etc.). 

\subsubsection*{Form Factor Made Simpler} On the other hand, however, the form factor seems to be somewhat simplified, making users easier to deal and utilize visualizations. One of the early forms of situated visualizations is the Touring Machine. This is, in large part, due to the advent of hand-held smartphones, a small powerful device that has ferociously become widely-used since its invention. Recently, high-performance, and light head-mounted displays (e.g., Microsoft HoloLens, Magic Leap) have been invented to provide a more authentic experience to augmented reality. This has also led to the rapidly increasing number of research in the past few years. 

\subsubsection*{Interactions Made Easier} Interactions too, have become easier than the past. The proportion of multiple interactions versus single interactions before 2010 have been 40\%, most of it being touch and physical. The change in such tendency may be down to the change in form factor - interactions are deeply influenced by the form factor. Those with touch-based interactions are those that utilize hand-held devices (most likely, smartphones) as their form factor.

\subsection{Limitations of Situated Analytics}
\label{sec:strengths-weaknesses}

Traditional visualizations are almost exclusively ex-situ, in that the analyst typically views the data divorced from the physical context and time where it was collected.
This has both benefits and limitations, as such ex-situ settings typically are conducted from the safety and comfort of an office or, sometimes, personal residence.
The opposite is true for SA, which by definition takes place in-situ and in real time.

Here we contrast in-situ visualizations with such ex-situ modes of visualization and enumerate the limitations for situated analytics systems found in the literature.

\paragraph{Field aspects.}

Proper situated analytics applications take place in the field and in the situation where the data is collected or analyzed (or both). 
This has unique impact on the user's performance:

    \begin{itemize}
        \item \textit{Strengths:} Situated analytics thrives in situated settings.
        \begin{itemize}
            \item[\adfrightarrowhead] \textit{Situatedness:} Data is displayed in the physical context where it is captured and/or needed.
                
            \item[\adfrightarrowhead] \textit{Cognitive load:} Using an in-situ visualization for situated analytics reduces the user's cognitive load because the platform and interface tends to be aligned with typical situated tasks.
            
            \item[\adfrightarrowhead] \textit{Spatial-centric tasks:} Compared to an ex-situ visualization, an in situ visualization is specifically aligned with spatial tasks that happen in the real world, thus minimizing context and attention switching.
            
            \item[\adfrightarrowhead] \textit{Simulation: } By embedding a virtual object into the real world context, users can test how the object interacts with the surrounding environment. This will help them make decisions from a spatial context, such as in designing in an urban environment, and shopping furnitures~\cite{schall09infravis,imottesjo18urbancobuilder}.
            
            \item[\adfrightarrowhead] \textit{Memory recall:} Understanding the data from a spatial context help users retain long-term memory. This would help them recall information better than when without being in spatial context~\cite{radu14augmented}. 
            
        \end{itemize}
    
        \item \textit{Weaknesses:} At the same time, there are significant challenges associated with venturing beyond the comfort of your office and into the field.
            \begin{itemize}

                \item[\adfrightarrowhead] \textit{Safety:} There are clear safety issues when navigating in a physical environment, such as being aware of traffic, physical obstacles, and other hazards.
                
                \item[\adfrightarrowhead] \textit{Distraction:} Navigating in a field setting exposes the user to more distractions than in an office.
    
                \item[\adfrightarrowhead] \textit{Eyes unavailable:} The field setting may mean that the user is unable to look at specific visual data projected in the world because their eyes are busy elsewhere (navigating, avoiding obstacles, looking at another person, etc).
                
                \item[\adfrightarrowhead] \textit{Wayfinding:} Finding a particular destination can be tricky in the best of times; it can be particularly difficult when also engaged in situated analytics tasks~\cite{dunser12outdoorsa}.

            \end{itemize}
        
    \end{itemize}
    
\paragraph{Technology aspects.}

Several aspects of situated analytics arise due to the unique software and hardware itself.
    This, again, can affect user performance:
    
    \begin{itemize}
        \item \textit{Strengths:} Because situated analytics equipment tends to be quite heterogeneous, different devices will have different capabilities.
            \begin{itemize}
                \item[\adfrightarrowhead] \textit{Smartphone-centric:} Many SA systems can take advantage of handheld AR technology using smartphones, making the tool accessible to large audiences.~\cite{williams17toarist, alqahtani17imapcampus, rollo17servar} 
                
               \item[\adfrightarrowhead] \textit{Hands-free (for certain devices):} SA systems that utilize head-mounted displays (i.e., not smartphones and tablets) enable users to work with their hands free~\cite{whitlock20fieldimmersive}.

            \end{itemize}
        \item \textit{Weaknesses:} Meanwhile, many of the drawbacks of these technologies arise from novel form factors and imperfect technology.
            \begin{itemize}
                \item[\adfrightarrowhead] \textit{Lack of familiarity:} Users are typically not familiar with specialized situated analytics equipment, such as head-mounted displays.
                
                \item[\adfrightarrowhead] \textit{Inaccurate location tracking:} With current positioning technology, regardless of the device, the location services often have errors larger than 2 meters.
                This limits the use of precise location as an input to situated analytics applications~\cite{dunser12outdoorsa}.

                \item[\adfrightarrowhead] \textit{Busy hands (for certain devices):} Some mobile devices require the user to interact with (and hold) the device using their hands. 
                This ties up the hands, making interacting with physical objects challenging.
                
                \item[\adfrightarrowhead] \textit{Expensive tools:} Specialized situated analytics hardware, such as head-mounted displays, are expensive and not easily accessible to a wide audience.
                
                \item[\adfrightarrowhead] \textit{Registration:} Properly detecting and aligning markers in the real world is difficult and often imprecise~\cite{imottesjo18urbancobuilder}.

                \item[\adfrightarrowhead] \textit{Sensitivity and robustness:} Many situated analytics devices are quite sensitive and require careful and frequent calibration.
                Because of the often immature technology used, the devices also tend to lack in robustness.
                For example, Microsoft HoloLens has optimal view two meters away from the virtual object~\cite{bach18hologram}.
                The view quality is reduced at near range.
                
                \item[\adfrightarrowhead] \textit{Heat and battery life:} Mobile devices all have limited battery life, and high energy consumption typically leads to high heat output.
                For example, the Magic Leap headset is notorious for easily overheating.\footnote{Ouch. Spoken from experience.}
                
                \item[\adfrightarrowhead] \textit{Limited text input:} Inputting text in a mobile setting is more difficult than when using a standard keyboard.
                
                \item[\adfrightarrowhead] \textit{Limited field of vision:} Even top-of-the-line head-mounted displays have limited view of the real world, and hand-held AR are even more reduced. 

                \item[\adfrightarrowhead] \textit{Accidental touches:} Using touch screens in the field is prone to accidental touches. 
                
            \end{itemize}
    \end{itemize}

\paragraph{Visualization aspects.}

Situated analytics excel at visualization tasks that are different from classical visualization systems, and, by the same token, are less suited to other tasks.
    
    \begin{itemize}
        \item \textit{Strengths:} The strengths of visualizations for situated analytics generally arise when the visual representations can be efficiently embedded in the real world.
            \begin{itemize}
            
                \item[\adfrightarrowhead] \textit{Spatial task affinity:} The immersive nature of typical situated analytics systems promote performing spatial tasks, such as arranging charts in space, moving around a visualization, and directly selecting data.

                \item[\adfrightarrowhead] \textit{Engagement:} Again, the immersive aspects of situated analytics tend to help users engage better with the data being visualized~\cite{abao18foodgo}. 
            
                \item[\adfrightarrowhead] \textit{Size estimation:} Situated analytics, by virtue of being embedded in the real world, has the benefit of being able to utilize real objects as visual cues to convey magnitude.
                Such spatial analogies have been shown to help concretize data~\cite{Kim2016}, and, when placed in situ, can help users better understand magnitudes~\cite{rollo17servar}.

            \end{itemize}
            
        \item \textit{Weaknesses:} By the same token, immersive visualizations can be vulnerable to certain weaknesses.
            \begin{itemize}
            
            \item[\adfrightarrowhead] \textit{Occlusion, distortion, navigation:} Despite recent developments in technology, issues on occlusion, distortion, and navigation still persist in 3D visualization~\cite{Elmqvist2008}. 
            
            \item[\adfrightarrowhead] \textit{Poor development ecosystem:} Designing AR-based situated analytics systems is usually more complicated than building desktop visual analytics systems because of the prevalence of exotic technology.
            Furthermore, while some immersive analytics toolkits exist~\cite{sicat19dxr, cordeil19iatk}, they are not yet widely accepted and used, and APIs for immersive technologies are in general scattered and non-standardized.
            This increases the burden of developing such systems. 
            
            \end{itemize}
    \end{itemize}
    
    
    
Traditional visualizations are almost exclusively ex-situ, in that the analyst typically views the data divorced from the physical context and time where it was collected.
This has both benefits and limitations, as such ex-situ settings typically are conducted from the safety and comfort of an office or, sometimes, personal residence.
The opposite is true for SA, which by definition takes place in-situ and in real time.

Here we contrast in-situ visualizations with such ex-situ modes of visualization and enumerate the limitations for situated analytics systems found in the literature.

\paragraph{Field aspects.}

Proper situated analytics applications take place in the field and in the situation where the data is collected or analyzed (or both). 
This has unique impact on the user's performance:

    \begin{itemize}
        \item \textit{Strengths:} Situated analytics thrives in situated settings.
        \begin{itemize}
            \item[\adfrightarrowhead] \textit{Situatedness:} Data is displayed in the physical context where it is captured and/or needed.
                
            \item[\adfrightarrowhead] \textit{Cognitive load:} Using an in-situ visualization for situated analytics reduces the user's cognitive load because the platform and interface tends to be aligned with typical situated tasks.
            
            \item[\adfrightarrowhead] \textit{Spatial-centric tasks:} Compared to an ex-situ visualization, an in situ visualization is specifically aligned with spatial tasks that happen in the real world, thus minimizing context and attention switching.
            
            \item[\adfrightarrowhead] \textit{Simulation: } By embedding a virtual object into the real world context, users can test how the object interacts with the surrounding environment. This will help them make decisions from a spatial context, such as in designing in an urban environment, and shopping furnitures~\cite{schall09infravis,imottesjo18urbancobuilder}.
            
            \item[\adfrightarrowhead] \textit{Memory recall:} Understanding the data from a spatial context help users retain long-term memory. This would help them recall information better than when without being in spatial context~\cite{radu14augmented}. 
            
        \end{itemize}
    
        \item \textit{Weaknesses:} At the same time, there are significant challenges associated with venturing beyond the comfort of your office and into the field.
            \begin{itemize}

                \item[\adfrightarrowhead] \textit{Safety:} There are clear safety issues when navigating in a physical environment, such as being aware of traffic, physical obstacles, and other hazards.
                
                \item[\adfrightarrowhead] \textit{Distraction:} Navigating in a field setting exposes the user to more distractions than in an office.
    
                \item[\adfrightarrowhead] \textit{Eyes unavailable:} The field setting may mean that the user is unable to look at specific visual data projected in the world because their eyes are busy elsewhere (navigating, avoiding obstacles, looking at another person, etc).
                
                \item[\adfrightarrowhead] \textit{Wayfinding:} Finding a particular destination can be tricky in the best of times; it can be particularly difficult when also engaged in situated analytics tasks~\cite{dunser12outdoorsa}.

            \end{itemize}
        
    \end{itemize}
    
\paragraph{Technology aspects.}

Several aspects of situated analytics arise due to the unique software and hardware itself.
    This, again, can affect user performance:
    
    \begin{itemize}
        \item \textit{Strengths:} Because situated analytics equipment tends to be quite heterogeneous, different devices will have different capabilities.
            \begin{itemize}
                \item[\adfrightarrowhead] \textit{Smartphone-centric:} Many SA systems can take advantage of handheld AR technology using smartphones, making the tool accessible to large audiences.~\cite{williams17toarist, alqahtani17imapcampus, rollo17servar} 
                
               \item[\adfrightarrowhead] \textit{Hands-free (for certain devices):} SA systems that utilize head-mounted displays (i.e., not smartphones and tablets) enable users to work with their hands free~\cite{whitlock20fieldimmersive}.

            \end{itemize}
        \item \textit{Weaknesses:} Meanwhile, many of the drawbacks of these technologies arise from novel form factors and imperfect technology.
            \begin{itemize}
                \item[\adfrightarrowhead] \textit{Lack of familiarity:} Users are typically not familiar with specialized situated analytics equipment, such as head-mounted displays.
                
                \item[\adfrightarrowhead] \textit{Inaccurate location tracking:} With current positioning technology, regardless of the device, the location services often have errors larger than 2 meters.
                This limits the use of precise location as an input to situated analytics applications~\cite{dunser12outdoorsa}.

                \item[\adfrightarrowhead] \textit{Busy hands (for certain devices):} Some mobile devices require the user to interact with (and hold) the device using their hands. 
                This ties up the hands, making interacting with physical objects challenging.
                
                \item[\adfrightarrowhead] \textit{Expensive tools:} Specialized situated analytics hardware, such as head-mounted displays, are expensive and not easily accessible to a wide audience.
                
                \item[\adfrightarrowhead] \textit{Registration:} Properly detecting and aligning markers in the real world is difficult and often imprecise~\cite{imottesjo18urbancobuilder}.

                \item[\adfrightarrowhead] \textit{Sensitivity and robustness:} Many situated analytics devices are quite sensitive and require careful and frequent calibration.
                Because of the often immature technology used, the devices also tend to lack in robustness.
                For example, Microsoft HoloLens has optimal view two meters away from the virtual object~\cite{bach18hologram}.
                The view quality is reduced at near range.
                
                \item[\adfrightarrowhead] \textit{Heat and battery life:} Mobile devices all have limited battery life, and high energy consumption typically leads to high heat output.
                For example, the Magic Leap headset is notorious for easily overheating.\footnote{Ouch. Spoken from experience.}
                
                \item[\adfrightarrowhead] \textit{Limited text input:} Inputting text in a mobile setting is more difficult than when using a standard keyboard.
                
                \item[\adfrightarrowhead] \textit{Limited field of vision:} Even top-of-the-line head-mounted displays have limited view of the real world, and hand-held AR are even more reduced. 

                \item[\adfrightarrowhead] \textit{Accidental touches:} Using touch screens in the field is prone to accidental touches. 
                
            \end{itemize}
    \end{itemize}

\paragraph{Visualization aspects.}

Situated analytics excel at visualization tasks that are different from classical visualization systems, and, by the same token, are less suited to other tasks.
    
    \begin{itemize}
        \item \textit{Strengths:} The strengths of visualizations for situated analytics generally arise when the visual representations can be efficiently embedded in the real world.
            \begin{itemize}
            
                \item[\adfrightarrowhead] \textit{Spatial task affinity:} The immersive nature of typical situated analytics systems promote performing spatial tasks, such as arranging charts in space, moving around a visualization, and directly selecting data.

                \item[\adfrightarrowhead] \textit{Engagement:} Again, the immersive aspects of situated analytics tend to help users engage better with the data being visualized~\cite{abao18foodgo}. 
            
                \item[\adfrightarrowhead] \textit{Size estimation:} Situated analytics, by virtue of being embedded in the real world, has the benefit of being able to utilize real objects as visual cues to convey magnitude.
                Such spatial analogies have been shown to help concretize data~\cite{Kim2016}, and, when placed in situ, can help users better understand magnitudes~\cite{rollo17servar}.

            \end{itemize}
            
        \item \textit{Weaknesses:} By the same token, immersive visualizations can be vulnerable to certain weaknesses.
            \begin{itemize}
            
            \item[\adfrightarrowhead] \textit{Occlusion, distortion, navigation:} Despite recent developments in technology, issues on occlusion, distortion, and navigation still persist in 3D visualization~\cite{Elmqvist2008}. 
            
            \item[\adfrightarrowhead] \textit{Poor development ecosystem:} Designing AR-based situated analytics systems is usually more complicated than building desktop visual analytics systems because of the prevalence of exotic technology.
            Furthermore, while some immersive analytics toolkits exist~\cite{sicat19dxr, cordeil19iatk}, they are not yet widely accepted and used, and APIs for immersive technologies are in general scattered and non-standardized.
            This increases the burden of developing such systems. 
            
            \end{itemize}
    \end{itemize}

\paragraph{Summary.} 

While most of the above strengths and weaknesses are well-understood in practice and well-documented in the literature, it is still true that many questions remain on the tradeoffs between sensemaking conducted ex-situ vs.\ in-situ (situated). 
Given our above review, we now set out to empirically study these tradeoffs in more detail.
We discuss this study in the following section.


\section{Discussion}
\label{sec:dicsussion}

We discuss future 

\subsection{\sungbok{safety issues}}

\begin{itemize}
    \item inaccurate technology, linear perspective (prediction, display in visualizations)
    \item Hololens - fixed eyesight
    \item Car, Phone view, Unfixed eyesight
\end{itemize}

\subsection{\sungbok{not much integration with ML techniques}}

\begin{itemize}
    \item Using machine learning techniques to make up for the insecure technology
    \item 
\end{itemize}

\subsection{\sungbok{Lacking real-time simulations.}}

\subsection{\sungbok{SA for accessibility}}

- In addition, there are 2 systems where audio is used as one of the integrations for SA. These systems are used. 



\subsection{Requirements for Situated Visualization}
\label{sec:requirements}

The scope of our meta-analysis are visualizations where the data are represented in its spatial context~\cite{white09sitelens}.
While a large part of situated visualizations deploy AR and other immersive techniques, situated visualizations, in its original and strict definition, are not only confined to 3D visualizations. 
To that end, we delimit \textit{visualization for situated analytics} to refer to examples that fulfill the following 4 requirements:


\subsection{Tasks}

Based on the research literature and existing commercial applications, we identify 8 main tasks that people tend to perform using situated visualizations. 

\begin{itemize}

\item \textbf{Information exploration (undirected):} One task of situated visualizations is providing unintentional contextual information about the location.
Google Maps, for example, automatically provides numerous types of information about the surrounding location (e.g., restaurants, gas stations, etc.).  

\item \textbf{Information seeking (directed):} Some situated analytics systems provide users contextual information for a specific purpose (e.g., highlighting the nutritional content of food products in a supermarket~\cite{abao18foodgo}).

\item \textbf{Memory and recall:} Humans have specialized spatial memory, allowing them to more easily memorize and recall information that can be placed in a spatial context~\cite{robertson98datamountain, radu14augmented}.

\item \textbf{Narrative construction:} Specialized situated analytics systems can support storytelling activity of users (e.g., crime scene investigation) by combining the spatial information with the advantage of being in-situ~\cite{datcu16csivis}. 

%Notification --> ??
\item \textbf{Situational awareness:} Another common task found in situated analytics systems is drawing the user's attention to specific features in the environment, such as highlighting a radar contact on a military HUD (or on T-1000's field of vision from the movie \textit{Terminator 2}), providing warnings when the user approaches a crime scene site, or flagging the arrival of an email in the user's inbox.

\item \textbf{Sensemaking (spatial sensemaking):} Sensemaking of spatial information is particularly useful in a situated setting, such as understanding walking patterns on a university campus, the impact of a new building on traffic, and the placement of buildings over time in a historic district. Sensemaking differs from narrative construction in that narrative construction tasks involve the specific spatial location when speculating stories, whereas spatial sensemaking discovers observable patterns within a situated setting. 

\item \textbf{View arrangement:} Arranging 3D object and data in a real world environment provides users the opportunity to try activities that were difficult or impossible in 2D~\cite{imottesjo18urbancobuilder}, such as virtually testing a piece of furniture product in the users' living room~\cite{ikea_app}. 

\item \textbf{Wayfinding (spatial navigation):} Wayfinding systems guide the user in physical navigation.
Advanced systems can even use information about the environment, such as traffic, crime rate, and time of day, to provide the optimal route to the destination.

\end{itemize}

\begin{comment}
\begin{table*}[tb]
  \caption{Taxonomy of papers collected about papers that utilize augmented reality in situated visualizations.}
  \label{tab:taxonomy_paperds}
  \scriptsize%
	\centering%
  
  \begin{tabu}{%
	r%
	*{14}{c}%
	*{2}{r}%
	}
	
  \toprule
  \multirow{17}{*}{hello}
   System & Year &   \rotatebox{80}{location} &   \rotatebox{80}{object} &   \rotatebox{80}{situ. events} &   \rotatebox{80}{placial} &   \rotatebox{80}{relative} &   \rotatebox{80}{fixed} &   \rotatebox{80}{sticky} & \rotatebox{80}{absolute} &   \rotatebox{80}{relative}  & \rotatebox{80}{2D}  & \rotatebox{80}{3D} & \rotatebox{80}{non-visual} & \rotatebox{80}{abstract} & \rotatebox{80}{map} & \rotatebox{80}{Sim. material}  \\
  \midrule
	A Touring Machine~\cite{feiner97touringmachine} & 1997 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
  Augmentable Reality~\cite{rekimoto98augmentable} & 1998 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 & 2 & 1 & 1 & 1 & 1 & 1 & 1 \\

  \midrule
  \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  \bottomrule
  \end{tabu}%
\end{table*}

\end{comment}

\section{Design Guidelines: Situated Visualization}
\label{sec:exploration}

The creation of design guidelines for spatially situated visualization has been identified as one of the ``Grand Challenges'' in IA~\cite{Ens2021}.
In this section, we present a collection of design recommendations for situated visualization based on our meta-analysis (Section~\ref{sec:design-space}).
Then, we consider the different ways in which visualization can be used for situated analytics based on our review of both academic and commercial SA systems.
Finally, we provide observable technical limitations situated analytics systems have.

\subsection{Recommendations for Design}
\label{sec:design_recommendations}
Based on our meta-analysis of existing implementations (Tables~\ref{tab:classification_1} and \ref{tab:classification_2}), we propose the following recommendations for design.

\subsubsection{\textbf{Interaction and Form Factor}}

\begin{itemize}
\item \textbf{Use overlays unless there is a good reason not to:} [...finish meee...]

\item \textbf{View arrangement is especially important for 3D embedded visualizations:} [...finish meee...]

\item \textbf{Use separated view maps for navigation tasks:} [...finish meee...]

\item \textbf{Exploit non-vision senses for situational awareness and wayfinding features:} [...finish meee...]

\item \textbf{Use 2D visualizations for narrative construction:} [...finish meee...]
\end{itemize}

\textbf{[...add some form factor items above...]}

\subsubsection{\textbf{Interaction Modality}}
\begin{itemize}

\item \textbf{Combine touch and physical interactions for view arrangement, narrative construction, and information exploration:} This could represent the ``drag and drop'' interaction parallel for a 3D view--the user touches something and physically moves around the space to arrange their view. It could also represent the press of a button to summon or dispel objects, touch and physical movement for interactions with markers, or any number of permutations. 
We cannot recommend, however, using physical interactions alone--there is a very clear shift away from that as the primary input in more recent implementations relative to older ones.

\item \textbf{Physical interactions are recommended for spatial sensemaking:} Tangible (physical) interactions tend to be viewed by researcher and user alike as an intuitive way to make sense of spatial information. 
This is often combined with other interaction types: Clicking a button to speak commands, using an analog lever with a brush gesture, \textbf{...} 
%as buttons, levers, switches and the like are more costly to implement and may even be seen as pass\'{e} by the developer. 
[...finish meee...]


[...finish meee...]

\item \textbf{Voice and spatial inputs should be used mainly for situational awareness elements of the view and for wayfinding tasks:} 
Similar to how the non-visual senses should be exploited for these types of features, the user's own non-visual interactions are best used in these cases. [...finish meee...]

\item \textbf{Pens or styluses are rarely used, but when they are, it is most often for spatial sensemaking and view arrangement:}
[...finish meee...]

\item \textbf{Markers are not often used as an interaction modality, but when they are it is most often for information seeking and view arrangement.} We suspect that the marker may act as a sort of 3D cursor in these instances.
[...finish meee...]
\end{itemize}


\subsubsection{\textbf{Navigation: Situating Means}}

\subsubsection {\textbf{Data Representation}}
%Sungbok will be adding this to the table %Although we do not explicitly review data representation in our meta-analysis table, [...]


%\begin{figure}[tbp]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/building-example.png}
%    \caption{Situated analytics showing the surrounding information about a real estate.
%    Public domain photo from Unsplash.}
%    \label{fig:building-example}
%\end{figure}

%\begin{figure}[tbp]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/baur-bus-ar}
%    \caption{Situated analytics presenting information related to a common everyday situation.
%    Photo by Osman Rana, augmented by Dominikus Baur (\url{https://bit.ly/2YmkHvI}).}
%    \label{fig:wayfinding-example}
%    \vspace{-0.15in}
%\end{figure}

%\begin{figure}[tbp]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/medical}
%    \caption{An operation room where the surgeon is using situated analytics technologies to conduct surgery.
%    Photo courtesy of the Augmentarium at University of Maryland (UMIACS).}
%    \label{fig:medical-example}
%\end{figure}

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\columnwidth]{figures/military}
%    \caption{Situated analytics being used in a military operation.
%    Photo courtesy of the Augmentarium at University of Maryland (UMIACS).}
%    \label{fig:military-example}
%    \vspace{-0.15in}
%\end{figure}


\subsection{Technical Limitations in Situated Analytics}
\label{sec:technical_limitations}

While there are numerous technical limitations with regards to situated analytics systems, we select several issues that are common to many of them.

\subsubsection{Inaccurate Location Information}
\label{subsec:inaccurate_location}

Inaccurate location information has long been an unsolved issue and is a bottleneck in  a number of systems.
GPS systems have limited accuracy for small device and do not work well indoors.
% While there are devices that provide highly accurate GPS information, they are usually so costly and heavy that it is not appropriate to be used as devices for situated analytics. 
Numerous situated analytics systems are based on mobile, hand-held devices and head-mounted displays. 
Normally, the accuracy of smartphones are within 5 meters, which is often not enough for tasks that require high levels of accuracy. 
A number of systems in our taxonomy~\cite{moller14indoornavigation, whitlock20fieldimmersive, dunser12ARoutdoornavigation, lee15boreholear} also discuss the lack of accuracy as their limitations. 
The issue of accurate object placement in the user's view has been identified as one of the ``Grand Challenges in Immersive Analytics''~\cite{Ens2021}.

That said, many works endeavor to supplement this deficiency using different methods, though they are not fully satisfactory.
Several systems support the use of markers to present the intended view. 
When the GPS sensor is not fully capable of capturing the exact location, users can manually take the photo of the marker, and the intended view will appear. 
However, although the intended view will appear, users may still have to turn around to retain a position where the view will precisely fit with their gaze view~\cite{cavallo16riverwalk}. 
Other alternative is the manual adjustment of wrong locations. 
This, however, becomes a burden for users each time they make adjustments.
Another work~\cite{lee12cityviewAR} provides a solution by making users less distracted by the lack of location accuracy by presenting compelling content on the user's field of vision that would outweigh the inaccuracy (e.g., virtual buildings placed in user's view). 
However, this cannot be an ultimate solution, as it is far from solving the problem. 
FieldView~\cite{whitlock20fieldimmersive} suggests an alternative approach that complements the lack of location accuracy by informing more precise location accuracy through localized connectivity. 

The possibility of a fully accurate GPS information in smartphones will contribute to a more developed situated analytics system.

\subsubsection{Perception Issues}
\label{subsec:occlusion_cluttering}

Perception barriers such as occlusion and clutter are well-known issues in immersive literature. 
Furthermore, when in-situ, environmental factors such as sun glare, moisture, and rain may also disturb the user's field of vision.

Occlusion arises when an obstacle blocks information from being properly shown. 
It makes users spend more time to view them than those that are not~\cite{guven06hypermediaar}.
Various attempts have been made to manage occlusion~\cite{Elmqvist2008}. 
A pilot study by Caggianese et al.~\cite{caggianese19arinformationseek} tackle occlusion by letting the user bring a faraway object in front of her to make it easy to view. 
Although the task of viewing occluded objects is made easier, users have to take the burden to manually bring the object in front of her. 
A construction visualization~\cite{behzadan15reviewarconstruction} deploys z-buffer algorithm to address the occlusion problem. 
Although this algorithm is relatively simple, it requires extra memory and computation, which can be a problem in a limited computing environment. 
In the work by Kotranza et al.~\cite{Kotranza09psychomotorcognitivetasks}, elements of visual feedback are rendered with partial transparency to prevent occlusion of the user's hands. 
This, however, causes another problem by making it hard for users to locate her fingertips. 
According to Henderson and Feiner~\cite{henderson11maintenancerepairar}, although occlusion is a serious view problem, people will still try to use the system if there are benefits that can outweigh the disadvantages. 

Cluttering is also another problem that many situated analytics systems face. 
Several works provide alternatives to deal with cluttering issues. 
For example, Zhao et al.~\cite{zhao19augmentedmuseum} argue that magnifying and distorting the targeted overlay is effective for data exploring and counting tasks.

In the field, the brightness of the sunlight disturbs the markers to be properly seen in user's field of vision~\cite{dunser12ARoutdoornavigation,king05viticulturesa}. 
Furthermore, the system can be sensitive to angles. 
For example, a long, flat view is critically vulnerable to being overwhelmed by bright sunlight. 

\subsubsection{Safety Issues}
\label{subsec:attention_division}

There are several situations in which situated analytics can be dangerous.
The first situation involves users being confronted with hardware or features that they are unfamiliar with.
Many situated analytics systems utilize head-mounted displays~\cite{jain15hmdvis, heller14mobaudioar}. 
However, head-mounted displays are not easily accessible and can be uncomfortable~\cite{guarese20augmentedsitvis}.
Hence, a proper level of training is required to achieve a high level of satisfaction and performance. 

Second is the ``inattentional'' blindness issue. 
When people are concentrating on a specific task, especially if the task demands greater attention, they are more likely to miss events and objects that take place within their field of vision~\cite{datcu16csivis}. 
In that respect, visual cues installed in users' field of vision can draw attention from users, which disturbs them from obtaining what is happening in their view~\cite{dixon13surgeons}. 
This can be a crucial problem when using situated analytics systems during operations where high level of concentration is required (e.g., airplane flying, surgery). 
To this end, careful design decisions must be made so that such distractions are made as minimal as possible.

The last, but not least, issue is the division of attention. 
Although contemporary smartphones and hand-held devices are able to reduce many tasks into the performance of a single interaction, conducting sophisticated operations often still requires multiple form factors. 
Such situated analytics systems are utilized in complex tasks, such as military operations~\cite{livingston02augmented} and crime scene investigations~\cite{datcu16csivis}. 
In order to deal with uncertainties, these systems try to incorporate multiple functions at the cost of multiple form factors. 
This can cause the division of attention between the smartphone user interface and the real environment.
For example, during a pilot collaborative crime scene investigation study~\cite{datcu16csivis}, investigators had to sustain higher level of concentration to keep up with situational awareness of other investigators. 
Such trade-off between form factor and task needs to be deliberately taken into account when designing situated analytics systems.

\section{The Future of Situated Analytics}
\label{sec:future_outlook}

Here we briefly discuss several directions for the future of situated visualizations.
We discuss the directions in three contexts: (1) the use of machine learning techniques, (2) privacy-aware situated analytics for collaborative environments, and (3) situated analytics for accessibility.

\subsection{Use of Machine Learning Techniques}

Artificial intelligence and machine learning have achieved breakthroughs in fields such as computer vision and natural language processing (NLP). 
Such techniques can also be used to benefit situated visualizations, although this is still a nascent research area. 

Deploying such techniques can support the user's analysis of their surroundings on the fly.
One application may be to use image segmentation and classification tasks to detect potentially interesting objects and scenes from the user's field of vision. 
We can also utilize optical character recognition (OCR) techniques to decipher text in the real world, and then use neural machine translation (NMT) techniques to provide translations from one language to another.
Machine learning can also be used to provide better location accuracy.
Hashemi et al.~\cite{hashemi16mlforlocaccuracy} provide a method to provide a more accurate map-segment matching accuracy using an artificial neural network (ANN). 

\subsection{Situated Collaboration: Frameworks, Security, and Privacy}

As MR technologies become increasingly common, there will be a corresponding need for collaboration between multiple situated analysts.
For example, the investigation of crime scenes and the excavation of archaeological sites would benefit from collaborative mechanisms. 
Thus, we think that future situated analytics frameworks will incorporate such collaborative features by default.

Of course, there are also serious security and privacy concerns in such collaborative settings.
When logging on a shared network, we normally use address-based group communication. 
This has potential dangers in that it discloses location information to a third party. 
Hence, to cope with such constraints, situated analytics systems must deploy privacy-aware techniques when enabling collaboration.

One possible suggestion would be the encounter-based communication (EbC) by Tsai et al.~\cite{tsai19enclosure}. 
EbC does not require users to disclose their identities by allowing them to authenticate as devices encountered at a given time and place. 
EbC can also be utilized between devices, or users that have never met and still retain a high level of privacy. 

\subsection{Situated Analytics for Accessibility}

Situated analytics can aid people with loss of sight or loss of hearing to better understand their surrounding space and any information related to it. 
There are systems that deploy sound patterns as cues to deliver such contextual information.
For example, Coughlan and Miele~\cite{coughlan17ar4vi} utilize a marker-based AR tool to provide the user the information about the object she is pointing at. 
They note that sound cues can support the task of providing information about the situation.
They also suggest that, with the development of techniques such as text-to-speech, speech-to-text, and OCR, such tools will help reduce a range of accessibility barriers. 

Situated analytics can also be beneficial to people with loss of hearing. 
For example, Jain et al.~\cite{jain15hmdvis} use visual cues on a head-mounted display to direct the user's attention to the person currently speaking in a multi-party conversation. 
Since visualization is an effective tool for presenting data in an intuitive manner, if designed effectively, it can provide fast and intuitive delivery of information surrounding the environment.



\begin{comment}


\textbf{Complex information about objects is, well, more complicated (than it is for location).} ---? 


\textbf{Does the research in C2 qualify as a different sub-field of visualization than the others?} --- ? 



\textbf{The visual metaphor of simulating real-world objects is a natural application of situated visualization.}

That is not to say that it is a superior one; rather, the authors of such systems found creating these simulations to be the most intuitive way of representing the data. 


\textbf{Non-visual data representations are a distinct type of situated analytics representation}

They have enough similarity with other types of situated visualizations, particularly in comparison with the outlier of C2, but are distinct enough to form their own cluster (C6).

\textbf{Simple vs. Complex, Location vs. Object: The differences that define clusters C1, C2, C3, and C4} %(( ANDREA HELP WITH THIS PLEASE -- I can't buy this ))

Four large clusters, C1 through C4, emerged in our analysis described in Section~\ref{sec:taxonomy_analysis}.
Clusters C2 and C3 use location as their situating triggers, while C1 and C4 are triggered by objects and contexts around the user.
Despite the apparent strength of the difference in our Figure~\ref{fig:clusters_formed} representing the dimensionality reduction of the features, implementations in C2 do have enough similarity to those in C3 and C4 that they can be considered to be on the border of falling into one of these other clusters. 
When we added a 64th paper to our cluster input dataset, it pulled several papers from cluster C2 to these other two clusters.
We believe that this occurs because \textbf{[could you explain this sungbok? No, I can't. I would not provide an analysis based on the displacement of the clusters, because they are, as you've seen very instable.]}


Of these four major clusters, all but C2 highlight that there is an intuition on the part  of system designers who are creating views anchored to the world to try to mimic the real objects in the users' surroundings.


C2 is a clear outlier on the horizontal axis of Figure~\ref{fig:clusters_formed}. 
Such strong distinction is possible because not only the systems are clearly distinguishable from other clusters, but also because they all share similar technical properties. 
The views in C2 are abstract and not simulated at all; the anchoring of the view for these systems is also divorced from the real world, being device-anchored screen, unlike many of the other situated visualization systems. 
So, what makes C2 so different? Use of mobile devices instead of HMD may be one factor.
In early studies, the systems in cluster C2 were device-anchored relative, while in later studies, they were device-anchored fixed--a view even less directly linked to the real world around the user.
In other words, over time, the views themselves of C2-type systems became even more divorced from the real world because, one could argue, views with positions strongly linked to the real world are not always superior for the use cases seen in C2.
\end{comment}

==> backups/scraps.tex <==
\subsection{Design Dimensions}
\label{subsec:design_dimensions}

We characterized the systems into 5 dimensions: (1) method of situating, (2) integration, (3) form factor, (4) interaction mode, and (5) navigation mode.
Each design dimension is a set, which means that individual systems may have multiple values; for example, a specific situated analytics system may both be wrist- and head-mounted.

\begin{itemize}
    \item \textbf{Situating Triggers} (ST): The criteria and mechanism for situating a visualization.
    \begin{itemize}
        \item[\adfrightarrowhead] \textit{geospatial coordinates}: The user's position in the world
        \item[\adfrightarrowhead] \textit{object recognizing/marker}: Specific items within the user's field of view, or markers indicating points of interest
    \end{itemize}
    
    \item \textbf{View Integration} (VI): How visualizations are presented and (sometimes) blended with imagery of the real world.
    \begin{itemize}
    
        \item[\adfrightarrowhead] \textit{map view}: data is provided in a separate geographical view. 
        
        \item[\adfrightarrowhead] \textit{separate view}: the real world and the visualizations are displayed in separate views. 
        
    \end{itemize}
    
    \item \textbf{Form Factor} (FF): The form of the physical device used for the situated analytics system.
    We distinguish devices by the position where they are mounted on the human body.
    \begin{itemize}
        \item[\adfrightarrowhead] \textit{mobile viewport (often, hand/wrist)}: the device is held in the user's hand or mounted on the user's wrist.
        \item[\adfrightarrowhead] \textit{world-mounted viewport}: the device is mounted in the world (e.g., in a dashboard or physical panel).
    \end{itemize}
    
    \item \textbf{Data \adfrightarrowhead ~Situated Representation Mapping (SM)}: The visual (or other sensory) marks, channels, and layouts used to represent data types in a situated environment 
    \begin{itemize}
        \item[\adfrightarrowhead] \textit{spatial}: location data, 3D models of objects
        \item[\adfrightarrowhead] \textit{abstract}: data not directly representing the user's spatial surroundings; may have temporal indexing (e.g., prices over time), or may represent features of surroundings that are directly linked to sensory input (e.g., temperature) 
        \begin{itemize}
            \item[\adfrightarrowhead] \textit{quantitative}: e.g., prices
            \item[\adfrightarrowhead] \textit{ordinal}: e.g., class rankings
            \item[\adfrightarrowhead] \textit{nominal}: e.g., descriptive text, categorical 
        \end{itemize}
    \end{itemize}

\end{itemize}






\subsection{Input \adfrightarrowhead ~Activity \adfrightarrowhead ~Output Mapping}


\begin{itemize}
    \item \textbf{Interaction Mode} (IM): The medium in which the user interacts with the presented visualizations and data.
    \begin{itemize}
        \item[\adfrightarrowhead] \textit{touch}: interaction by directly touching on the device (e.g., on a touch screen).
        
        \item[\adfrightarrowhead] \textit{button}: physical push buttons and dials on the device (e.g., keyboard, consoles).
        Touch-based keyboards do not belong to this category (rather to \textit{touch}), only physical keyboards. 
        
        \item[\adfrightarrowhead] \textit{gestural}: physical gestures or actions beyond touch and buttons, such as pointing, arm gestures, and leg movement.
        
        \item[\adfrightarrowhead] \textit{pen}: interaction using a pen-like object, e.g., pens and styli for tablets or ultra-mobile laptops.
        
        \item[\adfrightarrowhead] \textit{voice}: using speech input to control the interface.
                
        \item[\adfrightarrowhead] \textit{spatial}: interactions in space, such as when input is received by the user inhabiting a specific location, or by touching a specific object---whether real or augmented---in the world. 
        
        \item[\adfrightarrowhead] \textit{marker}: decoding a marker (e.g., fiducial marker) in the real world to interact with the system.
        
    \end{itemize}
    \item \textbf{Navigation Mode} (NM): How the user navigates between different visualizations.

    \begin{itemize}
        \item[\adfrightarrowhead] \textit{location}: navigate between visualizations through user movement (i.e., tracking location using GPS).
        
        \item[\adfrightarrowhead] \textit{gaze}: interacting and navigating with visualizations based on the user's head and gaze direction.
        
        \item[\adfrightarrowhead] \textit{pointing}: navigating between visualizations through user pointing gestures. 
        
        \item[\adfrightarrowhead] \textit{camera}: traversing visualization space using an on-device camera.
    
    \end{itemize}
    
    % \item \textbf{Activity} (AC): Activities that are performed using the system.
    %     \begin{itemize}
    %         \item [\adfrightarrowhead] \textit{simulation}: authentic imitation of a fictitious object/information into the real world (e.g, size estimation, modeling, etc.)
    %         \item [\adfrightarrowhead] \textit{analysis}: visual representations (e.g., bar charts, glyphs, etc.) to augment the analytical process.
    %         \item [\adfrightarrowhead] \textit{instructional}: direct guidance in the decision-making process of the user (e.g., path guidance, notifications, etc.).
    %         \item [\adfrightarrowhead] \textit{learning}: delivery of relevant facts and information for novel knowledge discovery (e.g., information about surrounding location, etc.).
    %         \item [\adfrightarrowhead] \textit{collaborative}: Enabling the contribution of multiple users in accomplishing the task.
    %     \end{itemize}

    \end{itemize}



While a large part of situated visualizations deploy AR and other immersive techniques, situated visualizations, in its original and strict definition, are not only confined to 3D visualizations. 
To that end, we delimit \textit{visualization for situated analytics} to refer to examples that fulfill the following 4 requirements:

\begin{itemize}

    \item[R1]\textbf{Data-driven:} The system should represent data and information. 
    \item[R2]\textbf{Visualization-based:} The system should represent the data in the form of visual components (e.g., charts, graphs, glyphs, etc.).
    
    \item[R3]\textbf{Mobile:} The user should be able to move around the real world and not be tethered to specific fixed equipment or displays.
    
    \item[R4]\textbf{Contextual/location-based:} The system should receive location information to present related spatial content to the user.

\end{itemize}


\section{OLD RESULTS}

\textbf{PREVIOUS DESCRIPTION--DEPRECATED}

\textbf{First cluster (12).} The first cluster has location as its situating trigger, data being depicted in 2D, and `abstract' in data abstraction. 
\textbf{Second cluster (10).} The second cluster also has location as its situating trigger, absolutely world-registered and fixed in device-anchored in view situatedness, and used abstract for data abstraction. 
\textbf{Third cluster (13).} The third cluster has absolute world-registered as view-situatedness, 3D as data depiction, and simulated material for data abstraction. 
\textbf{Fourth cluster (8).} The fourth cluster has object as situating trigger, fixed and device-anchored as view situatedness, 2D as its main data depiction, and abstract as data abstraction. 
\textbf{Fifth cluster (8).} Another cluster uses object as its situating trigger, 2D as data depiction, and abstract for data abstraction. 
\textbf{Sixth cluster (5).} The papers from the first cluster are 
\textbf{Seventh cluster (3).} The papers from the first cluster are 
\textbf{Eighth cluster (2).} The papers from the first cluster are 
\textbf{Ninth cluster (2).} The papers from the first cluster are 



\subsubsection{Integration}

In integration, unlike other dimensions, there are more multiple techniques than single ones (Fig.~\ref{fig:stat_paper_2}(c)).
Overall, 45 out of 70 systems have multiple techniques, and having two techniques is the most common number, observed in 26 of these 45 systems. 
The most common types of multiple integration technique is in combinations of map-sep-overlays---maps with separate overlays of the user's field of view---seen in 10 of these 45 systems.
Such visual integrations are usually deployed by systems where users are asked to navigate~\cite{williams17toarist, alqahtani17imapcampus, cavallo16riverwalk}.  
Another common type is the combination of overlay and embedded integrations, such as overlay-2D, overlay-3D, etc. 
2D- and 3D-embedded integrations are gaining popularity, arguably because they render a more authentic user experience and because various AR development toolkits (e.g., Apple ARKit, Google ARCore, etc.) make it more accessible for both programmers and consumers.
Among the 26 systems with the single technique, overlay is the most frequently seen technique, observed in 17 such systems. 
We argue that this is because overlays effectively provide textual information about objects in-situ.

Based on the graph shown in Fig.~\ref{fig:stat_paper_3}(c), integration exhibits two temporal trends. 
First, the number of systems with multiple techniques are rapidly increasing.
Second, systems with single technique are not the most common. 
Looking at recent data, those with multiple techniques are more prototypical of situated visualizations than those with single technique. 


\subsubsection{Form Factor}

In form factor, 52 out of 70 situated analytics systems have a single form factor, as shown in Fig.~\ref{fig:stat_paper_2}(a), of which 40 are hand-held. 
Hand-held devices exist mostly in the form of smartphones and tablets. 
Among those with multiple form factors, 11 out of 18 use both hand-held and head-mounted displays. 

Form factor tends to simplify as time progresses (Fig.~\ref{fig:stat_paper_3}(a)). 
We believe that this trend arises because having multiple form factors diverts user attention from the intended task~\cite{datcu16csivis}. 
%Hence, having simplified version will improve help users utilize the system easier. 
One of the early forms of situated visualizations is the Touring Machine~\cite{feiner97touringmachine}. 
Back then, computing a situated visualization with augmented reality required that the user carry around a backpack containing a laptop as a control center, and a GPS tracker for location information, while also wearing a head-mounted display to present an AR view.
However, the advent of a powerful, small-sized smartphones and high-performance, light head-mounted displays (e.g., Magic Leap and Microsoft HoloLens), the functions mentioned above can be performed within a single device. 
Since such devices are quickly spreading or have already spread to a wide audience, the number of research papers using these devices is also rapidly increasing.

\subsubsection{Interaction Mode (Object Manipulation Task)}

The interaction mode of most systems is also mostly composed of a single input modality.
Out of 70 systems, 50 are single-modality (Fig.~\ref{fig:stat_paper_2}(b)). 
Of the 50 single-mode systems, 27 use `touch' as their input modality. 
This result reflects the popularity of hand-held devices, such as smartphones and electronic tablets, as a form factor. 
The runner-up for single interaction modality is the `physical' modality~(11/50)---our shorthand for materially fabricated control mechanisms such as buttons or rollers---although the number stays constant throughout the observed years (1 or 2 per year), while the total number of systems are increasing. 
The fact that this modality comes in second may reflect the trend of physical interactions being replaced by `touch' and `gesture' modalities. 
The third place is `gesture'~(4/50).
Although gestures are not very common, the number of systems that use gestures are slowly on the increase. 

Multiple interaction modalities within a single system have become less frequent than they were in the past (Fig.~\ref{fig:stat_paper_3}(b)).
The proportion of multiple interaction modes in situated visualizations before 2010 was 50\% (11/22), whereas that after 2010 is down to 19\% (9/48). 
Types of multiple interaction modes mainly coexist with `touch' mode to supplement tasks that are not solely possible with smartphone touchscreens, such as `voice' and `marker.'

\subsubsection{Navigation Mode (Navigation Task)}

In navigation mode, 39 out of 70 systems have single and 31 have multiple modes, where 27 of the multiple modes are double, as shown in Fig.~\ref{fig:stat_paper_2}(d). 
Gaze~(25/70) and the combination of loc-gaze~(23/70) are the two most common forms of navigation modes. 
While numerous tasks can be conducted using only gaze view, there also exist significant number of sophisticated, multi-functional tasks that require high levels of location accuracy. 
However, gaze by itself is not enough to guarantee a stable, trustworthy location accuracy, many systems deploy location information to supplement the accuracy. 
Camera-based navigation is third place of usage of navigation mode (9/70). 
These systems are mainly marker-based systems. 

\begin{figure}[tbh]
    \centering
        \subfloat[Integration.]{
        \includegraphics[width=0.48\columnwidth]{figures/mps_integ.eps}
    }
    \subfloat[Form factor. ]{
        \includegraphics[width=0.48\columnwidth]{figures/mps_ff.eps}
    }
    \\
    \subfloat[Interaction mode.]{
        \includegraphics[width=0.48\columnwidth]{figures/mps_interact.eps}
    }
    \subfloat[Navigation mode.]{
        \includegraphics[width=0.48\columnwidth]{figures/mps_navi.eps}
    }
    \caption{\textbf{Evolution of modes per dimension.}
    Most dimensions have one modes per system as the most frequent ones, but in integration, two modes is the most frequent.}
    \label{fig:stat_paper_2}
\end{figure}

\begin{figure}[tbp]
    \centering
    \subfloat[Integration.]{
        \includegraphics[width=0.48\columnwidth]{figures/sac_integ.eps}
    }
    \subfloat[Form factor.]{
        \includegraphics[width=0.48\columnwidth]{figures/sac_ff.eps}
    }
    \\
    \subfloat[Interaction mode.]{
        \includegraphics[width=0.48\columnwidth]{figures/sac_interact.eps}
    }
    \subfloat[Navigation mode.]{
        \includegraphics[width=0.48\columnwidth]{figures/sac_navi.eps}
    }
    \caption{\textbf{Evolution of modes per system.}
    It is observable, except for integration, that the proportion of one mode per system is increasing.}
    \label{fig:stat_paper_3}
\end{figure}

\subsection{Characteristics of Situated Visualizations by Tasks}
\label{subsec:task_analysis}

Here we provide characteristics of situated visualizations by different tasks mentioned in the previous section. 

\begin{itemize}
    \item \textbf{Information exploration.}
    In numerous information exploration tasks, the most typical pattern between the 4 design dimensions is the combination of overlay as integration, hand-held as the form-factor, touch as interaction, and gaze as the navigation mode. 
    Systems for navigation (e.g., tourist applications~\cite{williams17toarist, alqahtani17imapcampus, cavallo16riverwalk} are presented with different integration pattern --- a combination of map, separate view, and overlaid information. 
    Systems such as~\cite{chen20staticvis} use 2D- and 3D-embedded visualizations to provide information.)
    
    \item \textbf{Information seeking.}
    In information seeking tasks, too, the most prevalent type of systems is the combination of overlaid information, hand-held device, touch interaction, and gaze view.
    This task is commonly exemplified in shopping applications.
    For example, FoodGo~\cite{abao18foodgo} provides nutritional information about products to incite users choose healthier products. 
    Another application, Horus Eye~\cite{elsayed16horuseye}, filters products by user's requirements. 
    
    \item \textbf{Memory and recall.}
    Systems classified as memory and recall support the task by providing guidance through embedded, or overlaid integration~\cite{sommerauer14matheducationar,chiang14arinquiryactivities}.
    Research show that using AR techniques has positive effects in augmenting cognition abilities~\cite{hou13using}.
    
    \item \textbf{Narrative construction.}
    In narrative construction tasks, user's field of vision is integrated mainly with overlays in combination with 2D and 3D embedded objects. 
    Their form factors are mostly hand-held with touch interaction, and location and gaze as their navigation modes. 
    The early form of systems that conduct narrative construction tasks used to have multiple form factors, but the latter ones are simplified to one form factor. 
    
    \item \textbf{Situational awareness.}
    Notification tasks are prevalent in automobiles for providing warnings of obstacles and collisions. 
    They use overlay as the integration, and heads-up displays (world) as their form factors.
    Voice and auditory signals are utilized to communicate between the driver and the car.
    
    \item \textbf{Spatial sensemaking.}
    Relatively older forms of situated visualizations used for spatial sensemaking tasks have overlay-hand-physical-gaze as their main values of the four dimensions.
    However, recent systems use 2D and 3D embedded objects and provide maps in separate views. 
    Their form factors are simplified. 
    While they mainly use both location and gaze view for navigation mode, they also sometimes use the camera for allocating virtual objects in a precise location. 
    
    \item \textbf{View arrangement.} % management?
    For view arrangement tasks, 2D and 3D objects are used with overlaid information as their integration. 
    The simulation of artificial object in 2D and 3D create an authentic user experience. 
    Early forms of view arrangement tasks are mainly designed for professional tasks such as manufacturing and the simulation of molecular models. They used multiple form factors. 
    However, the widespread use of smartphones paved the way for view arrangement tasks to be used by general audience (e.g., the IKEA Place app). 
    To render 2D and 3D objects in a precise location, many systems use cameras for navigation mode with fiducial markers.
    
    \item \textbf{Wayfinding.}
    Wayfinding tasks generally deploy map view in a separate view with overlays and sometimes sound cues in integration. 
    They are mainly hand-based, and use touch as their interaction mode, while some of them can interact using voice. 
    One notable pattern of wayfinding tasks is that they all have various methods of navigating (two, or sometimes three).
\end{itemize}





